Repairing Serializability Bugs in Distributed Database Programs via Automated Schema Refactoring

Serializability is a well-understood concurrency control mechanism that eases reasoning about highly-concurrent database programs. Unfortunately, enforcing serializability has a high-performance cost, especially on geographically distributed database clusters. Consequently, many databases allow programmers to choose when a transaction must be executed under serializability, with the expectation that transactions would only be so marked when necessary to avoid serious concurrency bugs. However, this is a significant burden to impose on developers, requiring them to (a) reason about subtle concurrent interactions among potentially interfering transactions, (b) determine when such interactions would violate desired invariants, and (c) then identify the minimum number of transactions whose executions should be serialized to prevent these violations. To mitigate this burden, in this paper we present a sound and fully automated schema refactoring procedure that transforms a program's data layout -- rather than its concurrency control logic -- to eliminate statically identified concurrency bugs, allowing more transactions to be safely executed under weaker and more performant database guarantees. Experimental results over a range of database benchmarks indicate that our approach is highly effective in eliminating concurrency bugs, with safe refactored programs showing an average of 120% higher throughput and 45% lower latency compared to the baselines.

==> figures/F_definition.tex <==
\begin {figure}[h]
 \begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lll}
    \mathcal{F} (q,\Sigma, \deltas{chsk}(R,f)) & \coloneq  &
    \mathcal{F}_\deltas{chsk}(q,\Sigma,R,f)
    \\
    \mathcal{F} (q,\Sigma, \deltas{addpk}(R,f)) & \coloneq  & \deltas{identity}
    \\
    \mathcal{F} (q,\Sigma, \deltas{intro}(R)) & \coloneq  & \deltas{identity}
    \\
    \mathcal{F} (q,\Sigma, \deltas{intro}(R,f,\rho)) & \coloneq  & 
    \mathcal{F}_\deltas{intro}(q,\Sigma,R,f,\rho)
\end{array}
  \end{mathpar}
\end{minipage}
\\[5mm]
\begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{llll}
    \mathcal{F}_\deltas{chsk}(q,\Sigma,R,f) \coloneq  \TODO{}
     & & & 
\end{array}
  \end{mathpar}
\end{minipage}
\\[5mm]
\begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{llll}
    \mathcal{F}_\deltas{intro}(q,\Sigma,R,f,\rho) \coloneq  \TODO{}
     & & & 
\end{array}
  \end{mathpar}
\end{minipage}

\caption{Definition of function $\mathcal{F}:(q\times\Delta\times\Sigma)\rightarrow\Gamma_r$}
\label{fig:syntax}
\end{figure}


==> figures/aau.tex <==
\def\scale1{0.35}


\begin {wrapfigure}{r}{.7in}
\begin{minipage}{.7in}
%
\begin{subfigure}[t]{0.24in}
  \begin{center}
\includegraphics[scale=\scale1]{figures/aau2.pdf}
\end{center}
\caption{}
\label{subfig:aau2}
\end{subfigure}
~%%%%%%%%%%%
\hfill
~%%%%%%%%%%%
\begin{subfigure}[t]{0.24in}
  \begin{center}
\includegraphics[scale=\scale1]{figures/aau3.pdf}
\end{center}
\caption{}
\label{subfig:aau3}
\end{subfigure}
~%%%%%%%%%%%
\hfill
~%%%%%%%%%%%
\begin{subfigure}[t]{0.24in}
  \begin{center}
\includegraphics[scale=\scale1]{figures/aau4.pdf}
\end{center}
\caption{}
\label{subfig:aau4}
\end{subfigure}

\caption{Refactoring schema as means to eliminate serializability anomalies.}
\label{fig:aau}
\end{minipage}
\end{wrapfigure}


==> figures/challenging_ref.tex <==
\begin{figure}[b]

\definecolor{pgrey}{rgb}{0.26,0.25,0.28}
\definecolor{javared}{rgb}{0.2,0.2,0.7} % for strings
\definecolor{javagreen}{rgb}{0.2,0.45,0.3} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\definecolor{weborange}{RGB}{0,75,0}

\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{Main-6},
  frame=single,
  rulecolor=\color{pgrey},
  keywordstyle=\color{black},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=left,
  %title=\footnotesize{getStudent(id)},
  xleftmargin=1.9em,
  framexleftmargin=1.25em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  tabsize=1,
  captionpos=b
  showspaces=false,
  showstringspaces=false,
  classoffset=2, % starting new class  
  morekeywords={return,update,into,select,set,from,where},
  keywordstyle=\color{sql},
  moredelim=[is][\textcolor{red}]{\%\%}{\%\%},
}


%
\begin{minipage}[b]{0.485\textwidth}
\begin{lstlisting}[]
remSt(id,course):
 x:=select co_st_cnt from COURSE where co_id=course//S6
 update COURSE set co_st_cnt=x.co_st_cnt-1  
    where co_id=course  //U5   
\end{lstlisting}
\end{minipage}
$\hstepl{}{\textsc{intro $v_2$}}{}$
\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{Main-7},
  frame=single,
  rulecolor=\color{pgrey},
  keywordstyle=\color{black},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=left,
  %title=\footnotesize{getStudent(id)},
  xleftmargin=1.9em,
  framexleftmargin=1.25em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  tabsize=1,
  captionpos=b
  showspaces=false,
  showstringspaces=false,
  classoffset=2, % starting new class  
  morekeywords={return,update,into,select,set,from,where},
  keywordstyle=\color{sql},
  moredelim=[is][\textcolor{red}]{\%\%}{\%\%},
}




\begin{minipage}[b]{0.48\textwidth}
\begin{lstlisting}[]
remSt(id,course):
 x:=select co_st_cnt from COURSE_ST_CNT_LOG 
    where co_id=course 
 insert into COURSE_ST_CNT_LOG values 
    (co_id=course,log_id=uuid(),co_st_cnt_log=-1)          
\end{lstlisting}
\end{minipage}




\caption{A challenging program refactoring step}
\label{fig:challenging_ref}
\end{figure}



==> figures/contain_definition.tex <==
\begin{figure}[h]
  \begin{minipage}{\textwidth}
        \begin{mathpar}
           \footnotesize
         \begin{array}{rlcl}
           \text{set of fields:}  & \eval{F\sqsubseteq F'}_\vc^\func{agg} & \coloneqq &  \forall f\in F.\; \exists f'\in F'.\; \eval{f\cong f'}_\vc^\func{agg} \\
           \text{set of update exps}  & \eval{U\sqsubseteq U'}_\vc & \coloneqq &  \forall f\in F.\; \exists f'\in F'.\; \eval{f\cong f'}_\vc^\func{agg} \\








           \text{sequence of queries:}  & \eval{Q\sqsubseteq Q'} & \coloneqq & \exists \vc,\func{agg}.\;
           (\forall {q\in Q, q'\in Q'}.\; \eval{q_\func{whc}\cong q'_\func{whc}}_{\vc.\theta})\wedge\\
                                   & & & (\forall q\in Q.\; \eval{q_\func{flds}\sqsubseteq \bigcup_{q'\in Q'}q'_\func{flds}}_\vc^\func{agg}) \\
           \text{command:}    & \eval{c_1;c_2\sqsubseteq c_1';c_2'}  & \coloneqq & \eval{c_1\sqsubseteq c_1'}\wedge \eval{c_2\sqsubseteq c_2'}\\
                              & \eval{\func{if}(e)\{c\}\sqsubseteq\func{if}(e')\{c'\}} & \coloneqq & \eval{e\cong e'}\wedge\eval{c\sqsubseteq c'} \\
                              & \eval{\func{print}(e)\sqsubseteq\func{print}(e')} & \coloneqq & \eval{e\cong e'}\\
           \text{transaction:}      & \eval{T(a^*)\{c\}\sqsubseteq T(a^*)\{c'\}} & \coloneqq & \eval{c\sqsubseteq c'}\\
         
         
         \end{array}
        \end{mathpar}

  \end{minipage}
    \caption{Program containment}
    \label{fig:contain_definition}
\end{figure}
~                


==> figures/eval_graph_overhead.tex <==
\begin{figure}[b]
\begin{minipage}{.45\textwidth}
  \includegraphics[scale=0.4]{figures/overhead.pdf}
\end{minipage}
~\hfill~
\begin{minipage}{.45\textwidth}
  \includegraphics[scale=0.4]{figures/overhead.pdf}
\end{minipage}
\caption{Performance comparison between versions of TPC-C and SEATS}
\label{fig:eval_graph_overhead}
\end{figure}



==> figures/eval_performance.tex <==
\begin {figure}[h]  
  
\begin{minipage}{0.95\textwidth}
\centering
\begin{subfigure}[b]{0.48\textwidth}  
  \includegraphics[width=\textwidth]{figures/eval/latency.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}  
  \includegraphics[width=\textwidth]{figures/eval/throughput.pdf}
\end{subfigure}
\end{minipage}

\caption{Performance overhead of refactoring Smallbank benchmark}
\label{fig:eval_performance}
\end{figure}





==> figures/eval_random.tex <==
\begin {figure}[t]  
\begin{minipage}{\textwidth}
\begin{footnotesize}
% TPC-C
\begin{subfigure}[b]{0.32\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/eval/smallbank_random.pdf}
  \caption*{SmallBank}
\end{subfigure}
%%
% SEATS
\begin{subfigure}[b]{0.32\textwidth}  
  \includegraphics[width=\textwidth]{figures/eval/seats_random.pdf}
  \caption*{SEATS}
\end{subfigure}
%%
% TICKET
\begin{subfigure}[b]{0.32\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/eval/tpcc_random.pdf}
\caption*{TPC-C}
\end{subfigure}
%%
\end{footnotesize}
\end{minipage}
  \caption{Number of anomalous access pairs in randomly 
  refactored benchmarks
}
  \label{fig:eval_random}
\end{figure}





==> figures/execution_example.tex <==
\def\scale1{0.295}


\begin {figure}[t]
\begin{minipage}{0.95\textwidth}
%
\begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
\includegraphics[scale=\scale1]{figures/running_example_execution_1.pdf}
\end{center}
%\caption{}
\label{subfig:execution_example1}
\end{subfigure}
~%%%%%%%%%%
\hfill
~%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
\includegraphics[scale=\scale1]{figures/running_example_execution_2.pdf}
\end{center}
%\caption{}
\label{subfig:execution_example2}
\end{subfigure}
~%%%%%%%%%%%
\hfill
~%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
\includegraphics[scale=\scale1]{figures/running_example_execution_3.pdf}
\end{center}
%\caption{}
\label{subfig:execution_example3}
\end{subfigure}
\caption{Executions of programs introduced in figure \ref{fig:running_example}}
\label{fig:execution_example}
\end{minipage}
\end{figure}


==> figures/fix_example_getSt.tex <==
\begin{figure}[h]


\definecolor{pgrey}{rgb}{0.26,0.25,0.28}
\definecolor{javared}{rgb}{0.2,0.2,0.7} % for strings
\definecolor{javagreen}{rgb}{0.2,0.45,0.3} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\definecolor{weborange}{RGB}{0,75,0}

\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{Main-6},
  frame=single,
  rulecolor=\color{pgrey},
  keywordstyle=\color{black},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=left,
  %title=\footnotesize{getStudent(id)},
  xleftmargin=1.9em,
  framexleftmargin=1.25em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  tabsize=1,
  captionpos=b
  showspaces=false,
  showstringspaces=false,
  classoffset=2, % starting new class  
  morekeywords={return,update,into,select,set,from,where},
  keywordstyle=\color{sql},
  moredelim=[is][\textcolor{red}]{\%\%}{\%\%},
}


%
\begin{minipage}[b]{0.9\textwidth}
\begin{lstlisting}[]
getSt(id):
  x := select * from STUDENT where st_id = id              //S1
  y := select em_addr from EMAIL where em_id = x.st_em_id  //S2
  z := select co_avail from COURSE where co_id=x.st_co_id  //S3
\end{lstlisting}
\end{minipage}

$\hstepl{}{v_1}{}$

\lstset{language=Java, backgroundcolor=\color{Main-6}}

\begin{minipage}[b]{0.9\textwidth}
\begin{lstlisting}[]
getSt(id):
  x := select * from STUDENT where st_id = id                      //S1
  y := select st_em_addr from STUDENT where st_em_id = x.st_em_id  //S2'
  z := select co_avail from COURSE where co_id=x.st_co_id          //S3
\end{lstlisting}
\end{minipage}

$\hstepl{}{v_2}{}$

\begin{minipage}[b]{0.9\textwidth}
\begin{lstlisting}[]
getSt(id):
  x := select * from STUDENT where st_id = id                      //S1
  y := select st_em_addr from STUDENT where st_em_id = x.st_em_id  //S2'
  z := select st_co_avail from STUDENT where st_co_id=x.st_co_id   //S3'
\end{lstlisting}
\end{minipage}

%\lstset{language=Java, backgroundcolor=\color{Main-7}}
%
%\begin{minipage}[b]{0.9\textwidth}
%\begin{lstlisting}[]
%getSt(id):
%  x := select * from STUDENT where st_id = id    //RS1
%\end{lstlisting}
%\end{minipage}
  
\caption{Refactoring steps of $\func{getSt}$}
\label{fig:fix_example_getSt}
\end{figure}



==> figures/fix_example_setSt.tex <==
\begin{figure}[h]


\definecolor{pgrey}{rgb}{0.26,0.25,0.28}
\definecolor{javared}{rgb}{0.2,0.2,0.7} % for strings
\definecolor{javagreen}{rgb}{0.2,0.45,0.3} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\definecolor{weborange}{RGB}{0,75,0}

\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{Main-6},
  frame=single,
  rulecolor=\color{pgrey},
  keywordstyle=\color{black},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=left,
  %title=\footnotesize{getStudent(id)},
  xleftmargin=1.9em,
  framexleftmargin=1.25em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  tabsize=1,
  captionpos=b
  showspaces=false,
  showstringspaces=false,
  classoffset=2, % starting new class  
  morekeywords={return,update,into,select,set,from,where},
  keywordstyle=\color{sql},
  moredelim=[is][\textcolor{red}]{\%\%}{\%\%},
}


%
\begin{minipage}[b]{0.8\textwidth}
\begin{lstlisting}[]
setSt(id,name,email):
  x := select st_em_id from STUDENT where st_id=id       //S4
  update STUDENT set st_name=name where st_id=id         //U1
  update EMAIL set em_addr=email where em_id=x.st_em_id  //U2         
\end{lstlisting}
\end{minipage}

$\hstepl{}{v_1}{}$


\begin{minipage}[b]{0.8\textwidth}
\begin{lstlisting}[]
setSt(id,name,email):
  x := select st_em_id from STUDENT where st_id=id             //S4
  update STUDENT set st_name=name where st_id=id               //U1
  update STUDENT set st_em_addr=email where st_em_id=x.st_em_id  //U2'         
\end{lstlisting}
\end{minipage}

%\lstset{  backgroundcolor=\color{Main-7}}
%
%\begin{minipage}[b]{0.8\textwidth}
%\begin{lstlisting}[]
%setSt(id,name,email):
%  update STUDENT set st_name=name, st_em_addr=email where st_id=id  
%\end{lstlisting}
%\end{minipage}
  
  
\caption{refactoring steps of $\func{setSt}$}
\label{fig:fix_example_setSt}
\end{figure}



==> figures/functions_table.tex <==
% settings
\setlength{\arrayrulewidth}{0.2mm}
\setlength{\tabcolsep}{4pt}

\def\arraystretch{0.99}
% table
\begin{center}
\begin{table}[h!]
  \caption{Functions used in the repair procedure}
  \label{fig:functions_table}
  \vspace{-1mm}
\centering
\begin{footnotesize}
{\rowcolors{2}{grey11}{white}
  \begin{tabular}{|l | l | l |} 
 \hline
    \rowcolor{grey9}
        \multicolumn{1}{|c}{\scriptsize Name} 
     &  \multicolumn{1}{c}{\scriptsize Type} 
     &  \multicolumn{1}{c|}{\scriptsize Description} \\ [0.1ex] 
 \hline
    $\func{try\_merge}$ & $P\times c \times c \rightarrow \func{Some}(P) $ &
    \tiny Refactors the given program by merging the input commands. Returns
    $\func{none}$ if merge is not possible
    \\ 
    %$\func{try\_split}$ & $P\times c \times \mathcal{P}(f) \rightarrow \func{Some}(P) $ 	          & warehouse	\\ 
    $\param{\func{try\_redirect}}$ & $P\times c \times R \rightarrow \func{Some}(P) $           & warehouse	\\ 
    $\param{\func{try\_trim}}$ & $P\times c\rightarrow \func{Some}(P)$          & warehouse	\\ 
 \hline
\end{tabular}
}
\end{footnotesize}
\end{table}
\end{center}


==> figures/iso_definitions.tex <==
\begin{figure}[t]
  \begin{minipage}{\textwidth}
    \begin{mathpar}
        \footnotesize
        \begin{array}{rlrl}
            \text{(11)}   & \multicolumn{3}{l}{\eval{e\cong e}} \\
            \text{(12)}   & \multicolumn{3}{l}{\eval{e\cong e'}\wedge \eval{e'\cong e''}\Rightarrow \eval{e\cong e''}} \\
            \text{(13)}   & \multicolumn{3}{l}{\eval{e \cong e'} \Rightarrow \eval{e'\cong e}}\\
            \text{(14)}   & \multicolumn{3}{l}{\eval{\phi[f]_{\func{exp}} \cong \func{at}^n(\func{proj}(f,\phi_\func{var}))}} \\
            \text{(15)}   & \eval{ \func{at}^1(\func{proj}(f,v)) \cong \func{at}^n(\func{proj}(f',v'))}  & \coloneqq &
            \exists_V.\; \eval{\func{whc}(v)\cong \func{whc}(v')}_{V} \wedge
            V.\rho=\func{any} \wedge V.\delta(f)=f' \\
            \text{(16)}   & \eval{ \func{at}^1(\func{proj}(f,v)) \cong \func{sum}(\func{proj}(f',v'))}  & \coloneqq &
            \exists_V.\; \eval{\func{whc}(v)\cong \func{whc}(v')}_{V} \wedge
            V.\rho=\func{sum} \wedge V.\delta(f)=f' \\
            \text{(17)}   & \eval{\phi\cong \phi'}_V & \coloneqq  &
            \forall_{f\in
              V.\theta_\func{dom}}.\;\eval{\phi[f]_\func{exp}\cong
                              \phi'[\theta(f)]_\func{exp}}\\
            \end{array}
        \end{mathpar}
  \end{minipage}
  \caption{Isomorphism on expressions and where clauses}
    \label{fig:iso_definitions}
\end{figure}
~                


==> figures/iso_judgement.tex <==
\def\horizontalSpace{1mm}  
\begin{figure}[h]
  \begin{minipage}{\textwidth}
    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
      \centering
%
%
%\begin{minipage}[t]{.12\textwidth}
%\ruleLabel{1}
%$$
%\RULE{
%\\
%}
%% ------------------------------------------------------------------------------------------------
%{
%V \vdash e\equiv e
%}
%$$
%\end{minipage}
%
%
%\hfill
%
%
%
%\begin{minipage}[t]{.13\textwidth}
%\ruleLabel{2}
%$$
%\RULE{
%  V \vdash e\equiv e'
%}
%% ------------------------------------------------------------------------------------------------
%{
%V \vdash e'\equiv e
%}
%$$
%\end{minipage}
%
%
%
%
%
%\hfill
%
%
%
%%
%
%\begin{minipage}[t]{.25\textwidth}
%\ruleLabel{3}
%$$
%\RULE{
% V \vdash e\equiv e'
%  \quad
% V \vdash e'\equiv e''
%}
%%% ------------------------------------------------------------------------------------------------
%{
%V \vdash e\equiv e''
%}
%$$
%\end{minipage}
%%
%%
%\hfill
%
%
%
%%
%
\begin{minipage}[t]{.4\textwidth}
\ruleLabel{1}
$$
\RULE{
  \\
 e = \phi[f]_\func{exp}
 \qquad
 e' = \func{at}^{e''} (\func{proj}(f,\phi_\func{var})
}
%% ------------------------------------------------------------------------------------------------
{
  \func{eq}(e,e',V)
}
$$
\end{minipage}
%
%
%
%
%
%
%
%
\hfill
%
%
%
%
%
%%
%
%
%
%
\begin{minipage}[t]{0.58\textwidth}
\ruleLabel{2}
$$
\RULE{
  e= \func{proj}(f,x))
  \qquad
  e'= \func{at}^{e''} (\func{proj}(f',x')
  \\
(R,\_,\theta,\delta,\func{any})\in V
\qquad
\delta(f) = f'
\qquad
\func{eq}(x_\func{whc},x'_\func{whc},\theta,V)
}
%% ------------------------------------------------------------------------------------------------
{
  \func{eq}(e,e',V)
}
$$
\end{minipage}
%
%
%
%
%
%
%
%
%
%
\\[\horizontalSpace]

%
%
%
%
%
%%
%
%
%
%
%
\begin{minipage}[t]{0.53\textwidth}
\ruleLabel{3}
$$
\RULE{
  e= \func{at}^1 (\func{proj}(f,x))
  \qquad 
  e' = \func{agg} (\func{proj}(f',x'))
  
  \\
(R,\_,\theta,\delta,\func{agg}) \in V
\quad
\delta(f) = f'
\quad 
\func{eq}(x_\func{whc},x'_\func{whc},\theta,V)
}
%% ------------------------------------------------------------------------------------------------
{
  \func{eq}(e,e',V)
}
$$
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
\hfill
%
%
%
%
%
%%
%
%%
%
%
%
%
%
\begin{minipage}[t]{0.37\textwidth}
\ruleLabel{4}
$$
\RULE{
  \mathsf{WF}(\phi)
  \qquad
  \mathsf{WF}(\phi')
  \qquad
  \mathsf{WF}(\theta)
\\
\forall_{f\in \theta_\func{dom}}.\; 
\func{eq}(\phi[f]_\func{exp}, \phi[\hat{\theta}(f)]_\func{exp}, V)
}
%% ------------------------------------------------------------------------------------------------
{
  \func{eq}(\phi,\phi',\theta,V)
}
$$
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
\hfill
%
%
%
%
%
%

%
%
%
\vspace{1mm}
\end{mdframed}
\end{minipage}
\caption{Implementation of predicate $\func{eq}\subseteq e\times e\times
  \mathcal{P}(v)$}
\label{fig:iso_judgement}
\end{figure}


==> figures/isomorphism.tex <==
\begin{figure}[t]
  \begin{minipage}{\textwidth}
    \begin{mathpar}
        \footnotesize
        \begin{array}{rlrl}
          (1) & \eval{c_1;c_2 \cong c_1';c_2'} & \coloneqq & \eval{c_1\cong c_1'} \wedge  \eval{c_2\cong c_2'} \\
          (2) & \eval{\func{if}(e) \{c\} \cong \func{if}(e')\{c'\}} & \coloneqq & \eval{c\cong c'}\wedge \eval{e\cong e'} \\
          (3) & \eval{\func{print}(e)\cong \func{print}(e')}& \coloneqq & \eval{e\cong e'}\\
          (4) & \eval{q_1;\dots;q_{n} \cong q'_1;\dots;q'_{m}} & \coloneqq 
                                    &  \exists_{V}.\; (\forall_{i\leq n}.
                                    \func{rel}(q_i)=V_\func{src})
                                    \wedge (\forall_{j\leq m}. \func{rel}(q'_j)=V_\func{dst})\; \wedge 
                                    \\
                                     &  &  &
                                      \forall_{i\leq n,j\leq m}.
                                      \eval{\func{whc}(q_i)\cong
                                      \func{whc}({q'_j})}_V\; \wedge\;
                                     \eval{q_1;\dots;q_{n} \cong q'_1;\dots;q'_{m}}_V \\
          (5) & \eval{q_1;\dots;q_{n} \cong q'_1;\dots;q'_{m}}_V  &\coloneqq & 
          \eval{\bigcup_{i\leq n} \func{fld}(q_i)\cong \bigcup_{j\leq m}
          \func{fld}(q'_j)}_V \quad\; \text{(for select queries)}\\
          (6) & \eval{q_1;\dots;q_{n} \cong q'_1;\dots;q'_{m}}_V  &\coloneqq & 
          \eval{\bigcup_{i\leq n} \func{upd}(q_i)\cong \bigcup_{j\leq m}
          \func{upd}(q'_j)} \qquad \text{(for non-select queries)} \\
          (7) & \eval{F\cong F'}_V & \coloneqq  &
          \eval{F\sqsubseteq F'}_V\wedge\eval{F'\sqsubseteq F}_V \\
          (8) & \eval{F\sqsubseteq F'}_V &\coloneqq & \forall_{f\in
          F}\,\exists_{f'\in F'}.\; (V.\delta(f)=f')\vee (V.\delta(f')=f)  \\
          (9) & \eval{U\cong U'} & \coloneqq  &
          \eval{U\sqsubseteq U'}\wedge\eval{U'\sqsubseteq U} \\
          (10) & \eval{U\sqsubseteq U'} & \coloneqq & \forall_{(f=e)\in
          U}\,\exists_{(f'=e')\in U'}.\; (f=f') \wedge \eval{e\cong e'}\\
        \end{array}
        \end{mathpar}
  \end{minipage}
  \caption{Isomorphism on commands}
    \label{fig:isomorphism}
\end{figure}


==> figures/modification_query.tex <==
\def\horizontalSpace{1mm}

\begin{figure}[t]
\begin{minipage}[b]{\textwidth}
    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.29\textwidth}
  \ruleLabel{comm-seq}
  $$
\RULE{
\hstepl{(c_1,M)}{v}{(c_1',M',\Delta)}
\\
\hstepl{(\Delta(c_2),M')}{v}{(c_2',M'',\Delta')}
}
%----------
{
  \hstepl{(c_1;c_2,M)}{v}{(c_1';c_2',M'',\Delta')}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.33\textwidth}
  \ruleLabel{comm-if}
$$
\RULE{
  \hstepl{(c_0,M)}{v}{(c'_0,M',\Delta)}
  \\
  c = \func{if}(e)\{c_0\}
  \qquad
  c' = \func{if}(e)\{c_0'\}


}
%----------
{
  \hstepl{(c,M)}{v}{(c',M'[c'\mapsto c],\Delta)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.33\textwidth}
    \ruleLabel{swap}
$$
\RULE{
  \neg\mathtt{depends}(c_1,c_2)
  \\
  c = c_1;c_2
  \qquad
  c' = c_2;c_1
}
%----------
{
  \hstepl{(c,M)}{\bot}{(c',M[c'\mapsto c],\lambda c.c)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.22\textwidth}
%    \ruleLabel{comm-aff}
%$$
%\RULE{
%  \\
%  \neg \mathtt{affects}(v,c)
%}
%%----------
%{
%  \hstepl{(c,M)}{v}{(c,M,\lambda c.c)}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
\begin{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.88\textwidth}
    \ruleLabel{merge}
$$
\footnotesize
\RULE{
  \phi\equiv_V\phi'
  \qquad
  c_1 = (x \!\coloneqq\! \sql{select} F \;\sql{from} R \;\sql{where} \phi)
  \qquad
  c_2 = (x' \!\coloneqq\! \sql{select} F' \;\sql{from} R \;\sql{where} \phi')
  \\
  c_3= (x \!\coloneqq\! \sql{select} F\cup F' \;\sql{from} R \;\sql{where}
  \phi)
  \qquad
  \Delta = 
  \lambda c. c[\forall f\in F'. \mathtt{proj}(f,x')/\mathtt{proj}(f,x)]
}
%----------
{
   \hstepl{(c_1;c_2,M)}{\bot}{(c_3,M[c_3\mapsto c_1;c_2],\Delta)
}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.98\textwidth}
    \ruleLabel{split}
$$
\footnotesize
\RULE{
  \neg\func{updated}(F,F')
  \qquad
  c_1= (x \!\coloneqq\! \sql{select} F\cup F' \;\sql{from} R \;\sql{where} \phi)
  \qquad
  c_2= (x \!\coloneqq\! \sql{select} F \;\sql{from} R \;\sql{where} \phi)
  \\
  c_3= (x' \!\coloneqq\! \sql{select} F' \;\sql{from} R \;\sql{where} \phi)
  \qquad 
  \Delta =
  \lambda c. c[\forall f\in F'. \mathtt{proj}(f,x)/\mathtt{proj}(f,x')]
}
%----------
{
  \hstepl{(c_1,M)}{\bot}{(c_2;c_3,M[c_2;c_3\mapsto c_1],\Delta)
}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.8\textwidth}
    \ruleLabel{redirect by $v$}
$$
\footnotesize
\RULE{
  c_1 = ( x\coloneqq \sql{select} F \;\sql{from} R \;\sql{where} \phi)
  \qquad
  v \in V
  \qquad
  \Delta = \lambda c.\; c[e/\func{redirect}(e,v)]
  \\
  c_2 = (x\coloneqq\sql{select} \{\func{redirect}(f,v)\,|\,f\in F\} \;\sql{from}
  R'\;\sql{where} \func{redirect}(\phi,v)) 
}
%----------
{
  \hstepl{(c_1,M)}{\bot}{(c_2,M[c_2\mapsto c_1],\Delta)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.97\textwidth}
%    \ruleLabel{redirect II}
%$$
%\footnotesize
%\RULE{
%  c_1 = ( x\coloneqq \sql{select} F \;\sql{from} R \;\sql{where} \phi)
%  \qquad
%   \Delta = \lambda c.\; c[\forall f\in F.\;
%   \func{at}^1\mathtt{(proj}(f,x))/\mathtt{sum(proj}(\delta(f),x))]
% \\
%   (R,R',\theta,\delta,\func{sum})\in V
%  \qquad  
%  \phi\equiv_\theta\phi'
%  \qquad
%  c_2 = (x\coloneqq\sql{select} \{\delta(f)\,|\,f\in F\} \;\sql{from} R'\;\sql{where} \phi') 
%  \qquad
% }
%----------
%{
%  \hstepl{(c_1,M)}{\bot}{(c_2,M[c_2\mapsto c_1],\Delta)}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{\textwidth}
    \ruleLabel{duplicate by $v$}
$$
\footnotesize
\RULE{
  c_1 = \sql{update} R \;\sql{set} U \;\sql{where} \phi
  \qquad
  c_2 = \sql{update} R' \;\sql{set}  \{\func{duplicate}(u,v)\,|\, u\!\in\! U\} \;\sql{where}
  \func{duplicate}(\phi,v)
    }
%----------
{
  \hstepl{(c_1,M)} 
  {v}
  {(c_1;c_2, M[c_1;c_2\mapsto c_1],\lambda c.c)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{minipage}[b]{0.72\textwidth}
%    \ruleLabel{duplicate III}
%$$
%\footnotesize
%\RULE{
%  q_1 = \sql{update} R_1\; \sql{set}  U_1 \;\sql{where} \phi_1
%  \qquad 
%  \phi_2 =  \phi_1[\forall f\in{\phi_1}_\func{flds}.\; f/\theta(f)] 
% \\
% U_2 = \{\delta(f)=\func{delta}(e,f) \,|\,(f=e)\in U\}
%\qquad
%U_2' = \{f=\phi_2[f]_\func{exp}\,|\, f\in {\phi_2}_\func{flds}\} 
%\\
%q_2 = \sql{insert}\sql{values} 
%U_2\cup U_2' \cup \{R_2\_uuid=\func{uuid}\}
%\; \sql{into} R_2
%  }
%%----------
%{
%  \hstepl{(\mathtt{sum},\delta,\theta),q_1} 
%{}
%    {q_1;q_2,\lambda c.c}
%}
%$$
%\end{minipage}












\begin{comment}
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.76\textwidth}
    \ruleLabel{duplicate II}
$$
\footnotesize
\RULE{
  q_1 = \sql{update} R_1 \;\sql{set} U \;\sql{where} \phi_1
  \quad
  q_2 = \sql{select} \func{pk}(R_2) \;\sql{from} R_2 \;\sql{as} v \;\sql{where} \phi_2
  \\ 
  \phi_2 =  \phi_1[\forall f\in{\phi_1}_\func{flds}.\; f/\theta(f)] 
  \qquad
  %{\phi_2}_\func{flds} \not\eq \func{pk}(R_2)
  \neg\func{full\_pk}(\phi_2)
  \\
  q_3 = \sql{update} R_2 \;\sql{set}  \{\delta(f)=e\,|\, (f=e)\in U\} \;\sql{where}
  \bigwedge_{f\in\func{pk}(R_2)}
  \mathtt{this}.f \;\IN\;\ \mathtt{proj}(f,v)
}
%----------
{
\hstepl{(\mathtt{any},\delta,\theta),q_1} 
{}
    {q_1;q_2;q_3,\lambda c.c}
}
$$
\end{minipage}
\end{comment}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{mdframed}
\end{minipage}
\caption{Semantics of refactoring database programs, cont'd}
\label{fig:modification_query}
\end{figure}


==> figures/modification_top.tex <==
\def\horizontalSpace{1mm}
\begin{figure}[h]
\begin{minipage}[b]{0.98\textwidth}
    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{minipage}[b]{0.65\textwidth}
   \ruleLabel{1}
$$
\RULE{
  \hstepl{c}{}{c'}
}
%----------
{
  \hstepl{
    (\set{R},\set{T}\cup\{t(\set{a})\{c;\func{return} e\}\})
  } 
  {}
    {
    (\set{R},\set{T}\cup\{t(\set{a})\{c';\func{return} e\}\})
    }
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}[b]{0.24\textwidth}
%   \ruleLabel{2}
%$$
%\RULE{
%  \hstepl{c_1}{}{c_1'}
%  \qquad
%  \hstepl{c_2}{}{c_2'}
%}
%----------
%{
%  \hstepl{
%    c_1;c_2
%  } 
%  {}
%    {
%    c_1';c_2'
%    }
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hfill
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.36\textwidth}
  \ruleLabel{2}
$$
\RULE{
  \hstepl{c_1}{}{c_1'}
}
%----------
{
  \hstepl{
  c;\func{if}(e)\{c_1\};c'
  }{}{
c;\func{if}(e)\{c_1'\};c'
}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{minipage}[b]{0.28\textwidth}
   \ruleLabel{3}
$$
\RULE{
  \neg\func{depends}(c_1,c_2)
}
%----------
{
  \hstepl{
    c;c_1;c_2;c'
  } 
  {}
    {
      c;c_2;c_1;c'
    }
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{minipage}[b]{0.48\textwidth}
   \ruleLabel{4}
$$
\RULE{
  {\param{\func{eq}(\phi,\phi',V)}}
  \\
  c_1 = (x \!\coloneqq\! \sql{select} \set{f} \;\sql{from} R \;\sql{where} \phi)
  \\
  c_2 = (x' \!\coloneqq\! \sql{select} \set{f'} \;\sql{from} R \;\sql{where} \phi')
  \\
  c_3= (x'' \!\coloneqq\! \sql{select} \set{f}\cup \set{f'} \;\sql{from} R \;\sql{where}
  \phi)
  \\
  c'' = c' [x.f_i/ x''.f_i][x'.f'_i/x''.f'_i]
}
%----------
{
  \hstepl{
    c;c_1;c_2;c'
  } 
  {}
    {
    c;c_3;c''
    }
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{minipage}[b]{0.48\textwidth}
   \ruleLabel{5}
$$
\RULE{
  {\param{\neg\func{upd}(\set{f},\set{f'})}}
  \\
  c_1= (x \!\coloneqq\! \sql{select} \set{f}\cup \set{f'} \;\sql{from} R \;\sql{where} \phi)
  \\
  c_2 = (x \!\coloneqq\! \sql{select} \set{f} \;\sql{from} R \;\sql{where} \phi)
  \\
  c_3 = (x' \!\coloneqq\! \sql{select} \set{f'} \;\sql{from} R \;\sql{where} \phi)
\\
  c'' = c' [x.f'_i/ x'.f'_i]
}
%----------
{
  \hstepl{
    c;c_1;c'
  } 
  {}
    {
    c;c_2;c_3;c''
    }
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{mdframed}
\end{minipage}
\caption{Program transformation semantics}
\label{fig:modification_top}
\end{figure}




==> figures/prog_ref_example_2.tex <==
\begin{figure}[t]

\definecolor{pgrey}{rgb}{0.26,0.25,0.28}
\definecolor{javared}{rgb}{0.2,0.2,0.7} % for strings
\definecolor{javagreen}{rgb}{0.2,0.45,0.3} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\definecolor{weborange}{RGB}{0,75,0}

\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{Main-6},
  frame=single,
  rulecolor=\color{pgrey},
  keywordstyle=\color{black},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=left,
  %title=\footnotesize{getStudent(id)},
  xleftmargin=1.9em,
  framexleftmargin=1.25em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  tabsize=1,
  captionpos=b
  showspaces=false,
  showstringspaces=false,
  classoffset=2, % starting new class  
  morekeywords={return,update,into,select,set,from,where},
  keywordstyle=\color{sql},
  moredelim=[is][\textcolor{red}]{\%\%}{\%\%},
}


%
\begin{minipage}[b]{\textwidth}
\begin{lstlisting}[]
regSt(id,course):
  x := select co_st_cnt from COURSE where co_id=course     //S1
  update COURSE set co_st_cnt=x.co_st_cnt+1  co_id=course  //U1   
  return (x.co_st_cnt)
\end{lstlisting}
\end{minipage}

$\hstepl{}{v_2}{}$

\lstset{language=Java,
  backgroundcolor=\color{Main-7},
}

\begin{minipage}[b]{\textwidth}
\begin{lstlisting}[]
regSt(id,course):
  x := select co_st_cnt from COURSE_ST_CNT_LOG where co_id=course //S1'                       
  insert into COURSE_ST_CNT_LOG values (co_id=course,log_id=uuid(),co_st_cnt_log=1)   //U1'
  return (sum(x.co_cnt_change))
\end{lstlisting}
\end{minipage}




\caption{A single program refactoring step}
\label{fig:prog_ref_example_2}
\end{figure}



==> figures/program_modification_syntax.tex <==
\begin {figure}[h]
 \begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
  \multicolumn{3}{c}{
    \stx{R,R'} \in {S}.\mathtt{RelationNames} \qquad
    \stx{f,f'} \in {S}.\mathtt{FieldNames} \qquad
 %   \stx{q,q'} \in P.\mathtt{Queries}
  } 
\\ \\
    %
\Gamma & \coloneqq &
\deltas{merge}()
\ALT 
\deltas{redirect}()
\ALT
\deltas{swap}()
%\\
%\Gamma_r & \coloneqq &
%\deltas{identity}
%\ALT 
%\deltas{atomicize}()
%\ALT
%\deltas{deatomicize}()
%\ALT
%\deltas{duplicate}()
%\\
%\Gamma & \coloneqq & \Gamma_s \ALT \Gamma_r
\end{array}
  \end{mathpar}
\end{minipage}
\caption{Syntax of possible modifications on commands of a given program
$P\in\mathbb{P}$ and a schema $S\in\mathbb{S}$}
\label{fig:syntax}
\end{figure}


==> figures/program_shrinking_semantics.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[h]
\begin{minipage}[b]{0.95\textwidth}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.32\textwidth}
  \ruleLabel{prog}
$$
\RULE{
  \hstepc{c}{}{c'}
}
%----------
{
  \hstepl{P\cup\{T(a)\{c\}\}} 
{}
{P\cup\{T(a)\{c'\}\}}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.32\textwidth}
    \ruleLabel{cond}
$$
\RULE{
  \hstepc{c_1}{}{c_2}
}
%----------
{
  \hstepl{c;\mathtt{if}(e)\{c_1\};c'} 
{}
{c;\mathtt{if}(e)\{c_2\};c'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.32\textwidth}
%    \ruleLabel{iter}
%$$
%\RULE{
%  \hstepc{c_1}{}{c_2}
%}
%----------
%{
%  \hstepl{c;\mathtt{iterate}(e)\{c_1\};c'} 
%{}
%{c;\mathtt{iterate}(e)\{c_2\};c'}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.1\textwidth}
    \ruleLabel{swap}
$$
\RULE{
  \neg\mathtt{depends}(q_1,q_2)
}
%----------
{
  \hstepl{q_1;q_2;c'} 
{}
    {q_2;q_1;c'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.1\textwidth}
    \ruleLabel{split I}
$$
\RULE{
  \hstepc{q_1;c}{}{q_2;q_3;c'}
}
%----------
{
  \hstepl{c;q_1;c'} 
{}
    {c;q_2;q_3;c'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.1\textwidth}
    \ruleLabel{merge I}
$$
\RULE{
  \hstepc{q_1;q_2;c}{}{q_3;c'}
}
%----------
{
  \hstepl{c;q_1;q_2;c'} 
{}
    {c;q_3;c'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.1\textwidth}
    \ruleLabel{redirect I}
$$
\RULE{
  \hstepc{q_1;c}{}{q_2;c'}
}
%----------
{
  \hstepl{c;q_1;c'} 
{}
    {c;q_2;c'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of database program refactoring}
\label{fig:schema_modification_semantics_sum}
\end{figure}




==> figures/program_shrinking_semantics_merge.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[h]
\begin{minipage}[b]{0.8\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\textwidth}
    \ruleLabel {merge II}
$$
\RULE{
  q_1\equiv \sql{select} F_1 \;\sql{from} R \;\sql{as} v_1 \;\sql{where} \phi
  \\
  q_2\equiv \sql{select} F_2 \;\sql{from} R \;\sql{as} v_2 \;\sql{where} \phi
  \\
  q_3\equiv \sql{select} F_1\cup F_2 \;\sql{from} R \;\sql{as} v_1 \;\sql{where} \phi
}
%----------
{
  \sstep{q_1;q_2;c} 
{}
{q_3;c[v_2/v_1]}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\textwidth}
    \ruleLabel {merge III}
$$
\RULE{
  q_1\equiv \sql{update} R \;\sql{set} U_1 \;\sql{where} \psi
  \\
  q_2\equiv \sql{update} R \;\sql{set} U_2 \;\sql{where} \psi
  \\
  q_3\equiv \sql{update} R \;\sql{set} U_1\cup U_2 \;\sql{where} \psi
}
%----------
{
  \sstep{q_1;q_2;c} 
{}
{q_3;c}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\textwidth}
    \ruleLabel {merge IV}
$$
\RULE{
  q_1\equiv \sql{select} F_1 \;\sql{from} R \;\sql{as} v_1 \;\sql{where}
  \mathtt{this}.k_1=e_1
  \\
  q_2\equiv \sql{select} \mathring{f} \;\sql{from} R \;\sql{as} v_2 \;\sql{where}
  \mathtt{this}.f=\mathtt{choose}(\mathtt{proj}(f,v_1),1)
  \\
  \deltas{intro}(R,\mathring{f},\rho)\in\mathcal{I}
  \qquad
  \rho=(\mathtt{id},R_s,\_,\phi)
  \qquad  
  \phi = \{R_s.k_s=R.f\}
  \\
  q_3\equiv \sql{select} F_1\cup \{\mathring{f}\} \;\sql{from} R \;\sql{as} v_1 \;\sql{where}
  \mathtt{this}.k_1=e_1
}
%----------
{
  \sstep{q_1;q_2;c} 
{}
{q_3;c[v_2/v_1]}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of query merging}
\label{fig:schema_modification_semantics_sum}
\end{figure}



==> figures/program_shrinking_semantics_redirect.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[h]
\begin{minipage}[b]{0.95\textwidth}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.51\textwidth}
    \ruleLabel{redirect II}
$$
\RULE{
  \deltas{intro}(R_d,\mathring{f},\rho) \in \mathcal{I}
  \qquad 
  \rho = (\mathtt{id},
  R_s,f_s,\phi)
  \\
  \phi=\{R_d.f_d=R_s.k_s\}
  \qquad
  \odot \in \{<, \leq, =,\neq, >, \geq,\IN\} 
  \\
  q\equiv \sql{select} f_s \;\sql{from} R_s \;\sql{as} v \;\sql{where}
  \mathtt{this}.k_s \odot e
  \\
  q'\equiv \sql{select} \mathring{f} \;\sql{from} R_d \;\sql{as} v \;\sql{where} 
  \mathtt{this}.f_d \odot e
}
%----------
{
  \sstep{q;c} 
{}
    {q';c[\mathtt{proj}(f_s,v)/\mathtt{proj}(\mathring{f},v)]}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.46\textwidth}
    \ruleLabel{redirect III}
$$
\RULE{
  \deltas{intro}(R_d,\mathring{f},\rho) \in \mathcal{I}
  \qquad 
  \rho = (\mathtt{sum},
  R_s,f_s,\phi)
  \\
  \deltas{intro}(R_d,k_d,\rho') \in \mathcal{I}
  \qquad 
  \rho' = (\mathtt{id},
  R_s,k_s,\phi')
  \\
  \phi'=\{R_d.f_d=R_s.k_s\} 
  \qquad
  \mathtt{PK}(f_d)
  \\
  q\equiv \sql{select} f_s \;\sql{from} R_s \;\sql{as} v \;\sql{where}
  \mathtt{this}.k_s = e
  \\
  q'\equiv \sql{select} \mathring{f} \;\sql{from} R_d \;\sql{as} v \;\sql{where}
  \mathtt{this}.k_d = e
}
%----------
{
  \sstep{q;c} 
{}
{q';c[\mathtt{proj}(f_s,v)/\mathtt{sum(proj}(\mathring{f},v))]}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of query redirection}
\label{fig:schema_modification_semantics_sum}
\end{figure}



==> figures/program_syntax.tex <==
\begin {figure}[h]
 \begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
  \multicolumn{3}{c}{
    \stx{T} \in \mathtt{TxnNames} \qquad
    \stx{a} \in \mathtt{Arguments} \qquad
    \stx{v} \in \mathtt{Variables} \qquad
<<<<<<< Updated upstream
    \mathtt{agg} \in \{\mathtt{sum,at^\mathbb{N}}\} 
  } 
  \\
  \multicolumn{3}{c}{
=======
    \stx{A} \in \{\mathtt{sum,max,min,count}\} \qquad
  } 
  \\
%  \multicolumn{3}{l}{
%    \stx{f,k} \in {S}.\mathtt{FieldNames} \qquad
%    \stx{R} \in S.\mathtt{RelationNames} \qquad
%  }
%  \\
  \multicolumn{3}{l}{
>>>>>>> Stashed changes
    \oplus \in \{+, -, \times, /\} \qquad
    \odot \in \{<, \leq, =,\neq, >, \geq,\IN\} 
  }\\
\\
    %
\stx{e} & \coloneqq &
\intt
\ALT 
\booll
\ALT
\stx{a}
\ALT \stx{e\oplus e}
\ALT \stx{e\odot e}
\ALT e \circ e
\ALT \stx{\mathtt{uuid}} 
\ALT \mathtt{iter} \ALT
\stx{\mathtt{proj}(v,{f})}
\ALT \stx{\mathtt{agg}(e)}
\\
<<<<<<< Updated upstream
u & \coloneq & {f} \leftarrow e
=======
\psi_{} &\coloneqq & 
\mathtt{this}.\hat{f} = e \ALT
\mathtt{this}.\hat{f} \;\IN\; e \ALT
\psi_{}\wedge \psi_{}
>>>>>>> Stashed changes
\\
\phi_{} &\coloneqq &
\mathtt{this}.f \odot e \ALT
\phi_{} \wedge \phi_{}
\\
\stx{q} & \coloneqq & 
<<<<<<< Updated upstream
\sql{select} {\set{f}}\; \sql{from} {R} \;\sql{as} \stx{v}\;
\sql{where} \stx{\phi} 
\ALT
\sql{update} {R}\;\sql{set} \set{u} \; \sql{where} \phi
\\
        & & \sql{insert} \sql{values} \set{u} \;\sql{into} {R}
\ALT
\sql{delete \;from} {R}\; \sql{where} \phi 
%\ALT \sql{atomic} q
 \\[0.2mm]
\stx{c} & \coloneqq &
\stx{q}
\ALT
\mathtt{if(e)}\{c\}
\ALT
\mathtt{iterate(e)\{c\}}
\ALT
c;c
\ALT \mathtt{eob}
\\
\mathbb{P} & \coloneqq & \stx{\set{T(a^*)\{c\}}}
=======
\sql{select} \stx{{f}^*}\; \sql{from} R \;\sql{as} \stx{v}\;
\sql{where} \stx{\phi} 
\ALT
\sql{update} R \;\sql{set} {(f=e)^*} \; \sql{where} \stx{\psi_{}}
\\
        & & \sql{insert} \sql{values} {e}^* \;\sql{into} R
\ALT
\sql{delete \;from} R\; \sql{where} \stx{\psi_{}} 
%\ALT \sql{atomic} q
 \\[0.2mm]
\mathbb{P} & \coloneqq & \stx{\overline{T({a}^*)\{q^*\}}}
>>>>>>> Stashed changes

\end{array}
  \end{mathpar}
\end{minipage}
\caption{Transactional programs running on a given schema
$S\in\mathbb{S}$}
\label{fig:program_syntax}
\end{figure}


==> figures/redirect_impl.tex <==
\def\horizontalSpace{1mm}  
\begin{figure}[t]
  \begin{minipage}{\textwidth}
    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
      \centering
\begin{minipage}[t]{.4\textwidth}
\ruleLabel{1}
$$
\RULE{
  v = (\_,\_,\_,\delta,\func{any})
  \\
  e = \func{proj}(f,x)
  \qquad
  e' = \func{proj}(\delta(f),x)
}
%% ------------------------------------------------------------------------------------------------
{
  \func{redirect}(e,x,v) \coloneqq e'
}
$$
\end{minipage}
%%
%
%
%
\hfill
%
%
%
%
\begin{minipage}[t]{.49\textwidth}
\ruleLabel{2}
$$
\RULE{
  v = (\_,\_,\_,\delta,\func{agg})
  \\
  e = \func{at}^1(\func{proj}(f,x))
  \qquad
  e' = \func{agg}(\func{proj}(\delta(f),x))
}
%% ------------------------------------------------------------------------------------------------
{
  \func{redirect}(e,x,v) \coloneqq e'
}
$$
\end{minipage}
%
%
%
\\[\horizontalSpace]
%
%
%
%
%
\begin{minipage}[t]{0.27\textwidth}
\ruleLabel{3}
$$
\RULE{
  v = (\_,\_,\theta,\_,\_)
  \\
  \phi' = \phi[\forall f\in\phi_\func{fld}.f/\hat{\theta}(f)]
}
%% ------------------------------------------------------------------------------------------------
{
  \func{redirect}(\phi,v) \coloneqq \phi'
}
$$
\end{minipage}
%
%
%
%
\hfill
%
%
%%
%
%\begin{minipage}[t]{0.25\textwidth}
%\ruleLabel{4}
%$$
%\RULE{
%  v = (\_,\_,\_,\delta,\_)
%}
%%% ------------------------------------------------------------------------------------------------
%{
%  \func{redirect}(f,v) \coloneqq \delta(f)
%}
%$$
%\end{minipage}
%%
%%
%%
%%
%\\[\horizontalSpace]
%
%
\hfill
%
%
%
%
\begin{minipage}[t]{0.27\textwidth}
\ruleLabel{4}
$$
\RULE{
  v = (\_,\_,\theta,\_,\func{any})
  \\
\phi' = \phi[\forall f\in\phi_\func{fld}.f/\hat{\theta}(f)]
}
%% ------------------------------------------------------------------------------------------------
{
  \func{duplicate}(\phi,v) \coloneqq  \phi'
}
$$
\end{minipage}
%
%
%
%\\[\horizontalSpace]
\hfill
%
%
%
\begin{minipage}[t]{0.43\textwidth}
\ruleLabel{5}
$$
\RULE{
  v = (\_,R',\theta,\_,\func{sum})
  \qquad 
  pk = \func{pk}(R')/\phi_\func{fld}
  \\
  \phi' =  
  \phi[\forall
  f\in\phi_\func{fld}.f/\hat{\theta(f)}]
  \wedge 
  (pk=\func{uuid})
}
%% ------------------------------------------------------------------------------------------------
{
  \func{duplicate}(\phi,v) \coloneqq \phi'
}
$$
\end{minipage}
%
%
%
\\[\horizontalSpace]
%
%
\begin{minipage}[t]{0.32\textwidth}
\ruleLabel{6}
$$
\RULE{
  v = (\_,\_,\_,\delta,\func{any})
  \\
U' = {(\delta(f)=e)\,|\, (f=e)\in U }\}
}
%% ------------------------------------------------------------------------------------------------
{
  \func{duplicate}(U,v) \coloneqq U'
}
$$
\end{minipage}
%
%
%
\hfill
%
\begin{minipage}[t]{0.67\textwidth}
\ruleLabel{7}
$$
\RULE{
  v = (\_,\_,\_,\delta,\func{sum})
  \quad
  \oplus \in \{+,-\}
  \\
  U = \{f=\func{at}^1(\func{proj}(f,x))\oplus e\}
  \qquad
U' = {(\delta(f)=e)\,|\, (f=(\oplus e))\in U }\}
}
%% ------------------------------------------------------------------------------------------------
{
  \func{duplicate}(U,v) \coloneqq U'\cup \{alive=\func{true}\}
}
$$
\end{minipage}
%
%
%
%
\vspace{1mm}
\end{mdframed}
\end{minipage}
\caption{Implementation of functions $\func{redirect}$ and $\func{duplicate}$}
\label{fig:redirect_impl}
\end{figure}


==> figures/schema_function_definitions.tex <==
\begin {figure}[h]
 \begin{minipage}{.85\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
    \deltas{chsk}(R,f) 
    & \coloneqq & 
    \lambda \mathbb{S}.\;
    \mathbb{S}[\mathbb{R}\mapsto \mathbb{R'} \ALT 
    \mathbb{R} = R(\_) \wedge
    \\ & & \quad 
    \mathbb{R'}=\mathbb{R}[(f,pk,\bot)\mapsto(f,pk,\top) \wedge 
    \\ & & \quad 
    (f',pk',\top)\mapsto (f',pk',\bot)]]
    \\
    \deltas{addpk}(R,f)
     & \coloneqq & 
    \lambda \mathbb{S}.\;
    \mathbb{S}[\mathbb{R}\mapsto \mathbb{R'} \ALT 
    \mathbb{R} = R(\_) \wedge
    \\ & & \quad 
    \mathbb{R'}=\mathbb{R}[(f,\bot,sk)\mapsto(f,\top,sk)]
    \\
    \deltas{intro}(\mathring{R}) 
    & \coloneqq & 
    \lambda \mathbb{S}.\;\mathbb{S}\cup\{\mathring{R}()\}
    \\
    \deltas{intro}(R_d,\mathring{f},\rho)
    & \coloneqq & 
    \lambda \mathbb{S}.\;
    \mathbb{S}[R_d(\seq{\mathbb{F}}) \mapsto R_d(\seq{\mathbb{F}};\mathring{f})]


    \\
\end{array}
  \end{mathpar}
\end{minipage}
\caption{Interpretation of refactorings as functions on schemas}
\label{fig:schema_function_definitions}
\end{figure}


==> figures/schema_modification_semantics_chsk.tex <==
\def\horizontalSpace{3mm}
\begin{figure}[h]
\begin{minipage}[b]{0.9\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.44\textwidth}
    \ruleLabel{IX}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q\equiv \sql{select} \overline{f}\; \sql{from} R \;\sql{as} v \;\sql{where} \phi
  \\
  \Sigma' = \Sigma[\mathtt{atmcVars\mapsto atmcVars}\cup\{v\}]
  \\
  q'\equiv \sql{atomic}\sql{select} \overline{f}\; \sql{from} R \;\sql{as} v \;\sql{where} \phi
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma')}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.52\textwidth}
    \ruleLabel{X}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q\equiv \sql{update} R \;\sql{set} \overline {f=e} \;\sql{where} \mathtt{this}.k \;\IN\; v
  \\
  v\in\Sigma.\mathtt{atmcVars}
  \\
  q'\equiv \sql{atomic} \sql{update} R \;\sql{set} \overline {f=e} \;\sql{where}
  \mathtt{this}.k \;\IN\; v
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.45\textwidth}
    \ruleLabel{XI}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q=\sql{delete}\sql{from} R \;\sql{where} \mathtt{this}.k \;\IN\; v
  \\
  v\in\Sigma.\mathtt{atmcVars}
  \\
  q'=\sql{atomic}\;\sql{delete}\sql{from} R \;\sql{where} \mathtt{this}.k \;\IN\; v
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.44\textwidth}
    \ruleLabel{XII}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q\equiv \sql{atomic}\sql{select} \overline{f}\; \sql{from} R \;\sql{as} v \;\sql{where} \phi
  \\
  \Sigma' = \Sigma[\mathtt{atmcVars\mapsto atmcVars}\backslash\{v\}]
  \\
  q'\equiv \sql{select} \overline{f}\; \sql{from} R \;\sql{as} v \;\sql{where} \phi
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma')}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.52\textwidth}
    \ruleLabel{XIII}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q\equiv \sql{atomic} \sql{update} R \;\sql{set} \overline {f=e} \;\sql{where} \mathtt{this}.k \;\IN\; v
  \\
  v\not\in\Sigma.\mathtt{atmcVars}
  \\
  q'\equiv \sql{update} R \;\sql{set} \overline {f=e} \;\sql{where}
  \mathtt{this}.k \;\IN\; v
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.47\textwidth}
    \ruleLabel{XIV}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \qquad
  \Delta = \deltas{chsk}(R,f')
  \\
  q=\sql{atomic}\sql{delete}\sql{from} R \;\sql{where} \mathtt{this}.k \;\IN\; v
  \\
  v\not\in\Sigma.\mathtt{atmcVars}
  \\
  q'=\sql{delete}\sql{from} R \;\sql{where} \mathtt{this}.k \;\IN\; v
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of database program expansion, cont'd}
\label{fig:schema_modification_semantics_chsk}
\end{figure}





==> figures/schema_modification_semantics_id.tex <==
\def\horizontalSpace{3mm}
\begin{figure}[h]
\begin{minipage}[b]{0.97\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.47\textwidth}
    \ruleLabel{duplicate I}
$$
\RULE{
  \hstepl{\phi}{\Psi}{\phi'}
  \\
  q\equiv \sql{update} R \;\sql{set} U \;\sql{where} \phi
  \\
  q'\equiv \sql{update} R' \;\sql{set} U' \;\sql{where} \phi'
  \\
  U\equiv \{u'|\hstepl{u}{\Psi}{u'}\wedge u\in U\}
  \qquad \mathtt{is\_pk}(\phi')
}
%----------
{
\hstepl{q} 
{\Psi}
    {q;q'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.52\textwidth}
    \ruleLabel{duplicate II}
$$
\RULE{
  \hstepl{\phi}{\Psi}{\phi'}
  \\
  q\equiv \sql{update} R \;\sql{set} U \;\sql{where} \phi
  \\
  q'\equiv \sql{select} \mathtt{PK}(R) \;\sql{from} R \;\sql{as} v \;\sql{where} \phi'
  \\
  q''\equiv \sql{update} R' \;\sql{set}  U' \;\sql{where}
  \bigwedge_{v\in\mathtt{PK}(R')}\mathtt{this}.k \;\IN\; \mathtt{proj}(k,v)
  \\
  U\equiv \{u'|\hstepl{u}{\Psi}{u'}\wedge u\in U\}
  \qquad \neg \mathtt{is\_pk}(\phi')
  %v
}
%----------
{
\hstepl{q} 
{\Psi}
    {q;q';q''}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.55\textwidth}
    \ruleLabel{duplicate III}
$$
\RULE{
  \hstepl{\phi}{\Psi}{\phi'}
  \\
  q\equiv \sql{update} R'\; \sql{set}  U \;\sql{where} \phi
  \\
  q'\equiv \sql{insert}\sql{values} \phi';uuid;U' \; \sql{into} R
  \\
  U\equiv \{u'|\hstepl{u}{\Psi}{u'}\wedge u\in U\}
}
%----------
{
  \hstepl{q} 
{\Psi}
    {q;q'}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{minipage}
\caption{Semantics of database program expansion, cont'd}
\label{fig:schema_modification_semantics_id}
\end{figure}





==> figures/schema_modification_semantics_sum.tex <==
\def\horizontalSpace{3mm}
\begin{figure}[h]
\begin{minipage}[b]{0.9\textwidth}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.55\textwidth}
    \ruleLabel{XXI}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \quad
  \Delta = \deltas{intro}(R,\mathring{f},\rho)
  \quad 
  \circ\in\{+,-\}
  \\
  \rho=(\mathtt{sum},R',f',{\phi}) 
  \quad
  \delta = \mathtt{choose}(\mathtt{proj}(f',v),1)
  \\
  q\equiv \sql{update} R'\; \sql{set} f'=\delta\circ e_1 \;\sql{where}
  \mathtt{this}.k'=e_2
  \\
  q'\equiv \sql{insert}\sql{values} e_2;\mathtt{uuid};\circ e_1 \; \sql{into} R
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q;q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.42\textwidth}
    \ruleLabel{XXII}
$$
\RULE{
  \mathtt{isAffected}(q,\Sigma,\Delta)
  \quad
  \Delta = \deltas{intro}(R,\mathring{f},\rho)
  \\
  \rho=(\mathtt{sum},R',f',{\phi}) 
  \\
  q\equiv \sql{insert} \sql{values} e_h;e_d;\seq{e_t} \;\sql{into} R'
  \\
  q\equiv \sql{insert} \sql{values} e_h;\mathtt{uuid},e_d \;\sql{into} R
}
%----------
{
  \step{(q,\Sigma)} 
{\Delta}
    {(q;q',\Sigma)}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of database program expansion, cont'd}
\label{fig:schema_modification_semantics_sum}
\end{figure}




==> figures/schema_modification_syntax.tex <==
\begin {figure}[H]
 \begin{minipage}{\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
  \multicolumn{3}{c}{
    \stx{R,R'} \in \mathbb{S}.\mathtt{RelationNames} \qquad
    \stx{f} \in  R \qquad f'\in R'
    \qquad
  } 
  \\
  \multicolumn{3}{c}{
    \mathring{R},\mathring{f} \in \mathtt{FreshNames} \qquad
    \stx{A} \in \{\mathtt{id,sum}\}
  } 
\\ \\
    %
\Delta & \coloneqq &
\deltas{chsk}(R,f)
\ALT \deltas{addpk}(R,f)
\ALT \deltas{intro}(\mathring{R}) \ALT
    \\ & & 
    \deltas{intro}(R', \mathring{f},\rho_{}) \ALT
 \Delta;\Delta \ALT \mathtt{skip}
\\
\rho_{} & \coloneqq & \mathtt{unique} \ALT (A,R,f,\phi) 
\\
\phi_{} &\coloneqq &
R'.f' = R.\hat{f}
\ALT
R'.\mathring{f} = R.\hat{f}
\ALT
\phi \wedge \phi
\end{array}
  \end{mathpar}
\end{minipage}
\caption{Possible refactorings on a given schema $\mathbb{S}$}
\label{fig:schema_modification_syntax}
\end{figure}


==> figures/schema_ref_example.tex <==
\begin{figure}[b]
\includegraphics[width=0.5\textwidth]{figures/schema_ref_example.pdf}
\caption{Two steps of schema refactoring}
\label{fig:schema_ref_example}
\end{figure}


==> figures/schema_syntax.tex <==
\begin {figure}[H]
 \begin{minipage}{\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
<<<<<<< Updated upstream
    {f} & \in & \mathtt{FieldNames}\\
    {R} & \in & \mathtt{RelationNames}\\
    \mathbb{R} & \coloneqq & {R}:\set{{f}}\\
    \mathbb{S} & \coloneqq & (\set{\mathbb{R}},\set{\mathbb{VC}})
=======
    R & \in & \mathtt{RelationNames}\\
    f & \in & \mathtt{FieldNames}\\
    b & \in & \{\top,\bot\}\\
    \mathbb{F} & \coloneqq & (f,b,b)\\
    \mathbb{R} & \coloneqq & R(\seq{\mathbb{F}})\\
    \mathbb{S} & \coloneqq & \overline{\mathbb{R}}
>>>>>>> Stashed changes
\end{array}
  \end{mathpar}
\end{minipage}
\caption{Database Schemas}
\label{fig:schema_syntax}
\end{figure}







==> figures/transformations.tex <==
\begin{figure}[h]
%    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
  \begin{minipage}{\textwidth}
  \footnotesize
\begin{itemize}
  
  \item[(comm)]
 $
    \begin{array}{llcl}
    (1) & \eval{V,c;c'}_v & \coloneqq & \eval{V,c}_v;\eval{V,c'}_v \\
    %(2) & \eval{\func{V,skip}}_v & \coloneqq & \func{skip} \\
    %(3) & \eval{\func{V,iterate}(e)\{c\}}_v & \coloneqq &
    %\func{iterate}(\eval{V,e}_v)\{\eval{V,c}_v\} \\
    (2) &  \eval{V,\func{if}(e)\{c\}}_v & \coloneqq &
    \func{if}(\eval{V,e}_v)\{\eval{V,c}_v\} \\
    \end{array}
    $
  
  \item [(whc)]
    $
     \begin{array}{llcl}
    (3) &   \eval{\phi\circ\phi'}_v & \coloneqq & \eval{\phi}_v\circ\eval{\phi'}_v \\
    (4) & \eval{\func{this}.f\odot e}_v & \coloneqq & \func{this}.f\odot \eval{e}_v \\
    \end{array}
    $

\item[(exp)] 
   $
    \begin{array}{llcl}
      (5) & \eval{V,\func{at}^e(x.f'')}_V & \coloneqq &
      \func{at}^{\eval{V,e}_v}(x.f'')\\
      (6) & \eval{V,\func{agg}(x.f'')}_V & \coloneqq &
      \func{agg}(x.f'')\\
 %     (7) & \eval{V,n}_V & \coloneqq & n \\
 %     (8) & \eval{V,a}_v & \coloneqq & a \\
 %     (9) & \eval{V,e\oplus e'}_v & \coloneqq & \eval{V,e}_v \oplus \eval{V,e'}_v\\
 %     (10) & \eval{V,e\odot e'}_v & \coloneqq &  \eval{V,e}_v \odot \eval{V,e'}_v \\
 %     (11) & \eval{V,e\circ e'}_v & \coloneqq &   \eval{V,e}_v \circ \eval{V,e'}_v\\
 %     (12) & \eval{V,\func{iter}}_v & \coloneqq & \func{iter}\\
  \end{array}
    $
  \item[(select)] 
    $
    \begin{array}{llcl}
      (7) & \eval{V,x:=\; \sql{select} f''\; \sql{from} {R}\ \sql{where} \stx{\phi}}_v
      & \coloneqq & (x:=\; \sql{select} {f''}\; \sql{from} {R}\ \sql{where}
  \eval{V,\phi}_v)\\
      (8) & \eval{V,x:=\; \sql{select} f''\; \sql{from} {R''}\ \sql{where} \stx{\phi}}_v
      & \coloneqq & (x:=\; \sql{select} {f''}\; \sql{from} {R''}\ \sql{where}
  \eval{V,\phi}_v)
%      \\
%      (11) & \eval{V,x:=\; \sql{select} f\; \sql{from} {R}\ \sql{where} \stx{\phi}}_v
 %     &  \coloneqq  & (x:=\; \sql{select} {f'}\; \sql{from} {R'}\ \sql{where}
 %     \param{\func{redirect}(V,\eval{\phi}_v,v)})
    \end{array}
    $
    

  \item[(update)]  $
    \begin{array}{llcl}
      (9) & \eval{V,\sql{update} R\; \sql{set} f''=e \;\sql{where}
  \phi}_v &  \coloneqq &  \sql{update} R\; \sql{set}
  f''=\eval{V,e}_v \;\sql{where}
  \eval{V,\phi}_v  \\
  (10) & \eval{V,\sql{update} R''\; \sql{set} f''=e \;\sql{where}
  \phi}_v &  \coloneqq &  \sql{update} R''\; \sql{set}
  f''=\eval{V,e}_v \;\sql{where}
  \eval{V,\phi}_v \\
 % (16) & \eval{V,\sql{update} R\; \sql{set} f=e \;\sql{where}
 % \phi}_v &\!\! \!\!\!\! \coloneqq & \!\!\! \!\!\!\sql{update} R'\; \sql{set} f'=\eval{e}_v \;\sql{where}
 % \param{\func{redirect}(V,\phi,v)}) \\
 % (17) & \eval{V,\sql{update} R\; \sql{set} f=e \;\sql{where}
 % \phi}_v & \!\!\! \!\!\! \coloneqq & \!\!\! \!\!\! \sql{update} R'\; \sql{set} \param{\func{duplicate}(V,f',\eval{e}_v)} \;\sql{where}
 % \param{\func{duplicate}(V,\eval{\phi}_v,v)})
    \end{array}
    $


\end{itemize}
\caption{Transformations triggered by a new value correspondence
$v=(R,R',f,f',\theta,\alpha)$}
  \label{fig:transformations}
\end{minipage}
%\end{mdframed}
\end{figure}




==> figures/vc_syntax.tex <==
\begin {figure}[H]
 \begin{minipage}{\textwidth}
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
    A & \in & \{\func{any},\func{sum}\}\\
    \Theta &\coloneqq & 
    \func{pk}({R}) \rightarrow \func{fld}({R'}) \\
    \Delta & \coloneqq & 
    \func{fld}({R}) \rightarrow \func{fld}({R'}) \\
    \mathbb{VC} & \coloneqq & 
    (A,\Delta,\Theta)
  \end{array}
  \end{mathpar}
\end{minipage}
\caption{Value correspondence}
\label{fig:vc_syntax}
\end{figure}







==> figures/whc_semantics.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[h]
\begin{minipage}[b]{\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.25\textwidth}
%    \ruleLabel {whc I}
%$$
%\RULE{
%  \hstepl{\phi_1}{\Psi_{}}{\phi_1'} \qquad
 % \hstepl{\phi_2}{\Psi_{}}{\phi_2'}
%}
%----------
%{
%  \hstepl{\phi_1\circ\phi_2}{\Psi_{}}{\phi_1'\circ\phi_2'}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\quad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.25\textwidth}
%    \ruleLabel {whc II}
%$$
%\RULE{
%  \Psi.\psi[f] = f'
%}
%%----------
%{
%  \hstepl{\mathtt{this}.f\odot e}{\Psi_{}}{\mathtt{this}.f'\odot e}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.3\textwidth}
    \ruleLabel {whc I}
$$
\RULE{
|\phi_1|=|\phi_2|
\\
\forall f \in \phi_1.\; \hstepl{\phi_1[f],\phi_2[f] }{}{\phi_1[f]}
}
%----------
{
  \hstepl{\phi_1,\phi_2}{}{\phi_1}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.37\textwidth}
    \ruleLabel {whc II}
$$
\RULE{
  e_1\cong e_2
\\
  \phi_1 \equiv \mathtt{this}.f\odot e_1
\qquad
\phi_2 \equiv \mathtt{this}.f\odot e_2
}
%----------
{
  \hstepl{\phi_1,\phi_2}{}{\phi_1}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.26\textwidth}
    \ruleLabel {whc III}
$$
\RULE{
  \phi_2.\mathtt{flds} = all Are Pks \\
  \mathtt{COMPONENTS}(\phi_2,v) \qquad 
  \func{whc}(v) = \phi_1
}
%----------
{
  \hstepl{\phi_1,\phi_2}{}{\phi_1}
}
$$
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\\[\horizontalSpace]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % \begin{minipage}[b]{0.29\textwidth}
 %   \ruleLabel {fld I}
%$$
%\RULE{
%  \Psi \equiv f=A(f')\; \sql{where} \_
%}
%%----------
%{
%  \hstepl{f}{\Psi}{f'}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.22\textwidth}
%    \ruleLabel {upd I}
%$$
%\RULE{
%  \hstepl{f}{\Psi}{f'}
%}
%%----------
%{
%  \hstepl{(f\leftarrow e)}{\Psi}{(f'\leftarrow e)}
%}
%$$
%\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\caption{Semantics of merging where clauses}
\label{fig:whc_semantics}
\end{figure}



==> related.tex <==
\section{Related Works}

==> sections/app_defs.tex <==
%
%A value correspondence $v = (R, R', f, f', \theta, \alpha)$ triggers a whole program transformation $\tau_v$.
%
%\begin{mathpar}
%\tau_v(\stx{x:=}\; \sql{select} {f}\; \sql{from} {R}\ \sql{where} \stx{\phi}) = \stx{x:=}\; \sql{select} {f'}\; \sql{from} {R'}\ \sql{where} redirect(\phi,v)
%\end{mathpar}
%
%$redirect(\phi,v)$ satisfies the following property, w.r.t. to a well-formed set of value correspondences $V$. (Note that $V$ does not include $v$, and corresponds to previous value correspondences):
%\begin{mathpar}
%\forall \Sigma, \Sigma', \Delta, \Delta'.\ \forall r \in R_{id}.\ \forall r' \in R'_{id}. \Sigma \preceq_V \Sigma' \wedge \Delta \preceq_V \Delta' \wedge \Sigma,\Delta,r, \phi \Downarrow true  \wedge r' \in \theta(r) \Rightarrow \\ \Sigma', \Delta', r',\ redirect(\phi,v) \Downarrow true 
%\end{mathpar}
%
%For SELECT queries to any other field or any other relation, the following transformation applies:
%$$
%\tau_v(\stx{x:=}\; \sql{select} {f''}\; \sql{from} {R''}\ \sql{where} \stx{\phi}) = \stx{x:=}\; \sql{select} {f''}\; \sql{from} {R''}\ \sql{where} \tau_v(\phi)
%$$
%
%For WHERE clauses, the following transformation is applicable:
%$\tau_v(\mathtt{this}.f \odot e ) = \mathtt{this}.f \odot \tau_v(e)$
%
%If $\alpha = any$, then,
%$\tau_v(\stx{\func{at}^e(x.f)}) = \stx(\func{at}^e(x.f'))$
%
%For an update command $q = \sql{update} {R}\;\sql{set} f = e \; \sql{where} \phi$, $\tau_v(q)$ must satisfy the following property:
%\begin{mathpar}
%\forall \Sigma, \Sigma', \Delta, \Delta'.\ \forall r \in R_{id}. \Sigma \preceq_V \Sigma' \wedge \Delta \preceq_V \Delta' \wedge \Sigma,\Delta,r, \phi \Downarrow true  \wedge \Sigma', \Delta', \tau_v(q) \rightarrow \Sigma'', \Delta',\mathtt{skip} \wedge \Delta, e \Downarrow n  \Rightarrow n = \alpha(\{m | r' \in \theta(r) \wedge \Sigma'', r', f' \Downarrow m \})
%\end{mathpar}
%
%
%\begin{definition}[Value Correspondence]
%A value correspondence from relation
%$R$ to relation $R'$ is defined a tuple $(R, R',
%\theta,\delta,\alpha)$ with the following components:
%\begin{enumerate*}[label=(\roman*)]
%  \item a \emph{record correspondence function}, denoted by
%    $\theta:R_\func{id}\rightarrow \mathcal{P}(R'_\func{id})$,
%    which relates
%    a record in $R$ to
%    a \emph{set} of corresponding records in $R'$,
%  \item a partial
%mapping from fields in $R$ to fields in $R'$, denoted by
%$\delta:\func{fld}(R)\rightharpoonup\func{fld}(R')$,
%and
%  \item a fold function on values,
%denoted by $\alpha: \mathcal{P}(\func{Val})\rightarrow \func{Val}$.
%\end{enumerate*}
%\end{definition}
%
%\begin{definition}[Database Containment Relation]
%A data-store state $\Sigma$ is
%contained in a data-store state $\Sigma'$ under a set of value correspondences $V$, (denoted by $\Sigma \preceq_{V} \Sigma'$)
%if
%\begin{mathpar} 
%\forall v=(R,R',\theta,\delta,\alpha).\ \forall_{r\in R_\func{id}}\, \forall_{f\in\delta_\func{dom}}.\; \Sigma,r(f)\Downarrow n \Rightarrow
%  \alpha(\{m\,|\,
%  r'\in \theta(r) \wedge \Sigma',r'(\delta(f))\Downarrow m\})=n
%  \end{mathpar}
%\end{definition}
%
%\begin{definition}[Execution History Refinement]
%An execution history $h'=(\Sigma', \Gamma')$ refines an execution history $h = (\Sigma, \Gamma)$ w.r.t. a well-formed set of value correspondences $V$ (denoted as $h \preceq_V h'$) if and only if 
%\begin{enumerate}
%\item There exists a bijective mapping $\omega:\Gamma_{\func{fin}} \rightarrow \Gamma'_{\func{fin}}$ such that $\forall \gamma \in \Gamma_{\func{fin}}.\ \gamma.\func{TxnName} = \omega(\gamma).\func{TxnName}$, $\gamma.\func{arg} = \omega(\gamma).\func{arg}$ and $\gamma.\func{ret}= \omega(\gamma).\func{ret}$
%\item $\Sigma \preceq_V \Sigma'$.
%\end{enumerate}
%\end{definition}
%
%\begin{definition}[Program Refinement]
%A program $P'$ is a refinement of program $P$ w.r.t. a well-formed set of value correspondences $V$,
%denoted by $P\preceq_V P'$,
%if and only if the following conditions hold:
%\begin{enumerate}
%  \item For any execution of $P'$, there is an execution of $P$, such that
%    former is a refinement of the latter, i.e.
%  $\forall_{h'\in\hist(P')} \exists_{h\in\hist(P)}.\; h \preceq_V h'$.
%\item For any serial execution of $P$, there is an execution of $P'$, such that
%    latter is a refinement of the former, i.e.
%  $\forall_{h \in \hist(P)_{\func{ser}}} \exists_{h' \in \hist(P')}.\; h \preceq
%  h'$.
%\end{enumerate}
%\end{definition}
%
%


==> sections/app_eval.tex <==
\section{Complete Evaluation Results}
\label{app:eval}






\begin {figure}[h]  
\begin{minipage}{0.4\textwidth}
\begin{footnotesize}
% TPC-C
\begin{subfigure}[h]{\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/eval/SmallBank.pdf}
 % \caption*{SmallBank}
\end{subfigure}
%%
% SEATS
\begin{subfigure}[h]{\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/eval/SEATS.pdf}
 % \caption*{SEATS}
\end{subfigure}
%%
% TICKET
\begin{subfigure}[h]{\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/eval/TPC-C.pdf}
%\caption*{TPC-C}
\end{subfigure}
%%
\end{footnotesize}
\end{minipage}
  \caption{Number of anomalous access pairs in randomly
  refactored programs
}
  \label{fig:eval_random2}
\end{figure}







\begin {figure*}[t]  
\begin{minipage}{\textwidth}
\begin{footnotesize}
% VA
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/seats_3.pdf}
  
\end{subfigure}
%%
% US
\begin{subfigure}[b]{0.33\textwidth}  
\includegraphics[width=\textwidth]{figures/evaluation/seats_2.pdf}
\end{subfigure}
%%
% GLOBAL
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/seats_1.pdf}
\end{subfigure}
% VA
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/seats_6.pdf}
\end{subfigure}
%%
% US
\begin{subfigure}[b]{0.33\textwidth}  
  \includegraphics[width=\textwidth]{figures/evaluation/seats_5.pdf} 
\end{subfigure}
%%
% GLOBAL
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/seats_4.pdf}
\end{subfigure}
%%
\end{footnotesize}
\end{minipage}
  \caption{Performance evaluation of SEATS benchmark}
  \label{fig:perf_eval}
\end{figure*}









\begin {figure*}[t]  
\begin{minipage}{\textwidth}
\begin{footnotesize}
% VA
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/tpcc_4.pdf}
  
\end{subfigure}
%%
% US
\begin{subfigure}[b]{0.33\textwidth}  
\includegraphics[width=\textwidth]{figures/evaluation/tpcc_3.pdf}
\end{subfigure}
%%
% GLOBAL
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/tpcc_2.pdf}
\end{subfigure}
% VA
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/tpcc_1.pdf}
\end{subfigure}
%%
% US
\begin{subfigure}[b]{0.33\textwidth}  
  \includegraphics[width=\textwidth]{figures/evaluation/tpcc_6.pdf}
\end{subfigure}
%%
% GLOBAL
\begin{subfigure}[b]{0.33\textwidth}  
\centering
  \includegraphics[width=\textwidth]{figures/evaluation/tpcc_5.pdf}
\end{subfigure}
%%
\end{footnotesize}
\end{minipage}
  \caption{Performance evaluation of TPC-C benchmark}
  \label{fig:eval_random}
\end{figure*}



==> sections/app_proofs.tex <==
Given a program $P$ and a value correspondence $v=$ $(R, R',$ $f, f', \theta, \alpha)$, let $\mathcal{V}^{\func{id}}_{v,P}$ be the set containing all identity value correspondences for all fields of all relations of $P$ except the fields $f,f'$ and the value correspondence $v$. The notation also generalizes for a set of value correspondences $V$ (i.e. $\mathcal{V}^{\func{id}}_{V,P}$ is the union of the set of all identity value correspondences for all fields of all relations of $P$ except the fields which are source and target fields in $V$, and the set of the value correspondence $V$). In accordance with the definitions in \autoref{sec:refactor}, here we define a containment relation between
sets of records as follows:
\begin{align*}
  X \sqsubseteq_V
  & X' ~~\equiv~~ \\
  &
    \forall (R,R',f,f',\theta,\alpha)\in V.\;
    \forall r\in R_\func{id}.\; r \in X_{id} \Leftrightarrow\\ & \theta(r) \cap X'_{\func{id}} \neq \emptyset \wedge \\
    & X(r.f)=\alpha(\{m\,|\,r'\in\theta(r) \cap X'_\func{id}~\wedge~ X'(r'.f')=m\})\\
\end{align*}

We begin the proofs by formalizing $\eval{.}$ and $R1-R3$ requirements in more detail. The transformation on select commands is defined as follows:
\begin{mathpar}
  \eval{c}_v = (x:=\,\sql{select} f'\; \sql{from} {R'}\ \sql{where}
  \func{redirect}(v, {\phi},)),
\end{mathpar}
 where  the function  $\func{redirect}: v \times \phi \rightarrow \phi$
 satisfies the following constraint:
 \ruleLabel{R1}
 \begin{equation*}
      %\tag{R1}
       \RULE{
         r\in R_\func{id}
 \qquad
   \Sigma\sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P}} \Sigma'
   \qquad
   \Delta\sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P}}\Delta'}
       {r \in \Sigma_{\func{id}} \wedge \Delta,\phi(\Sigma(r))\Downarrow \func{true} \Leftrightarrow
 \theta(r) \cap \{r' \in R'_\func{id}\,|\, r' \in \Sigma' \wedge
 \\
  \Delta',{\func{redirect}(v,\phi)}(\Sigma'(r')) \Downarrow \func{true}\} \neq \emptyset \wedge \\
 \Sigma(r.f) = \alpha(\{\Sigma'(r'.f')\ |\ r' \in \theta(r) \wedge \Delta',{\func{redirect}(v,\phi)}(\Sigma'(r')) \Downarrow \func{true}\})}
 \end{equation*}
 
 \ruleLabel{R2}
 \begin{equation*}
       \RULE{

       \Delta \sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P}} \Delta'
        
       }{
       \Delta, e \Downarrow n \Leftrightarrow \Delta',\eval{e}_v \Downarrow n
     }
     \end{equation*}

The redirect function takes a value correspondence and a WHERE clause, and returns another WHERE clause. The rule (R1) ensures that if the database state $\Sigma$ and local state $\Delta$ are contained inside $\Sigma'$ and $\Delta'$ respectively, then the output of SELECT query in the original program must be contained in the output of the SELECT query in the refactored program. A sufficient condition for this is that for every record $r$ in $\Sigma$ which satisfies the original WHERE clause $\phi$ (expressed as $\Delta,\phi(\Sigma(r))\Downarrow \func{true}$), there must be records in $\theta(r)$ that satisfy the new WHERE clause (that is returned by $redirect$), and that the values in the selected fields in the original record $r$ can be determined using the records in $\theta(r)$.

The rule (R2) simply says that if the local database state $\Delta$ is contained inside $\Delta'$, then any expression $e$ on $\Delta$ or $\Delta'$ must evaluate to the same value.

 For any command
 $c=\sql{update} R\ \sql{set} f=e\ \sql{where}\phi$ in the original program, which is
 affected by the newly added  $v=(R,R',f,f',\theta,\alpha)$, the refactored command is given by:
\begin{equation}
\eval{c}_v :=  \sql{update} R'\ \sql{set} f' = 
\\
\func{duplicate}(e,v)\ \sql{where} \func{duplicate}(\phi,v)
\end{equation}
The refactored command must satisfy the following property:
 \ruleLabel{R3}
  \begin{equation*}
 \RULE
 {
   \Sigma\sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P}} \Sigma' \qquad
   \Delta \sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P}} \Delta'
   \qquad
   \Sigma',\Delta',\llbracket c \rrbracket_v \rightarrow \Sigma'',\Delta',\func{skip}
   \qquad
   r\in R_\func{id}
 }
 {
  r \in \Sigma_\func{id} \wedge \Delta,\phi(\Sigma(r)) \Downarrow \func{true} \Leftrightarrow \{r' \in R'_\func{id}\ |\ r' \in \Sigma'_\func{id} \wedge  \\
  \Delta', \func{duplicate}(\phi,v)(\Sigma(r')) \Downarrow \func{true}\} \cap \theta(r) \neq \emptyset
  \\    \Delta,e\Downarrow n \Leftrightarrow \alpha(\{ \Sigma''(r'.f')  \,|\, r'\in\theta(r) \wedge r' \in \Sigma''_\func{id} \}) = n
 }
 \end{equation*}

The rule (R3) states that if the database state $\Sigma$ and local state $\Delta$ are contained inside $\Sigma'$ and $\Delta'$ respectively, and if the execution of the refactored UPDATE leads to the new database state $\Sigma''$, then for every record $r$ whose field $f$ is modified by the original UPDATE (modified to the valuation of the expression $e$), there must be records in $\theta(r)$ which must be modified by the refactored UPDATE, and that the modification in the original UPDATE (i.e. value of expression $e$) can be determined from the modified records obtained after the execution of the refactored UPDATE. This ensures that the original UPDATE is preserved by the refactored UPDATE. 

\begin{figure*}[h]
%    \begin{mdframed}[backgroundcolor=grey10,linecolor=grey10]
  \begin{minipage}{\textwidth}
  \footnotesize
\begin{itemize}
  
  \item[(comm)]
 $
    \begin{array}{llcl}
    (1) & \eval{c;c'}_v & \coloneqq & \eval{c}_v;\eval{c'}_v \\
    (2) & \eval{\func{skip}}_v & \coloneqq & \func{skip} \\
    (3) & \eval{\func{iterate}(e)\{c\}}_v & \coloneqq &
    (4)\func{iterate}(\eval{e}_v)\{\eval{c}_v\} \\
    (5) &  \eval{\func{if}(e)\{c\}}_v & \coloneqq &
    \func{if}(\eval{e}_v)\{\eval{c}_v\} \\
    \end{array}
    $
  
  \item [(whc)]
    $
     \begin{array}{llcl}
    (6) &   \eval{\phi\circ\phi'}_v & \coloneqq & \eval{\phi}_v\circ\eval{\phi'}_v \\
    (7) & \eval{\func{this}.f\odot e}_v & \coloneqq & \func{this}.f\odot \eval{e}_v \\
    \end{array}
    $

\item[(exp)] 
   $
    \begin{array}{llcl}
      (8) & \eval{\func{at}^e(x.f'')}_v & \coloneqq &
      \func{at}^{\eval{e}_v}(x.f'')\\
      (9) & \eval{\func{agg}(x.f'')}_v & \coloneqq &
      \func{agg}(x.f'')\\
      (10) & \eval{n}_v & \coloneqq & n \\
      (11) & \eval{a}_v & \coloneqq & a \\
      (12) & \eval{e\oplus e'}_v & \coloneqq & \eval{e}_v \oplus \eval{e'}_v\\
      (13) & \eval{e\odot e'}_v & \coloneqq &  \eval{e}_v \odot \eval{e'}_v \\
      (14) & \eval{e\circ e'}_v & \coloneqq &   \eval{e}_v \circ \eval{e'}_v\\
      (15) & \eval{\func{iter}}_v & \coloneqq & \func{iter}\\
  \end{array}
    $
  \item[(select)] 
    $
    \begin{array}{llcl}
      (16) & \eval{x:=\; \sql{select} f''\; \sql{from} {R}\ \sql{where} \stx{\phi}}_v
      & \coloneqq & (x:=\; \sql{select} {f''}\; \sql{from} {R}\ \sql{where}
  \eval{\phi}_v)\\
      (17) & \eval{x:=\; \sql{select} f''\; \sql{from} {R''}\ \sql{where} \stx{\phi}}_v
      & \coloneqq & (x:=\; \sql{select} {f''}\; \sql{from} {R''}\ \sql{where}
  \eval{\phi}_v)
%     \\
%      (18) & \eval{x:=\; \sql{select} f\; \sql{from} {R}\ \sql{where} \stx{\phi}}_v
%      &  \coloneqq  & (x:=\; \sql{select} {f'}\; \sql{from} {R'}\ \sql{where}
%     \param{\func{redirect}(\eval{\phi}_v,v)})
    \end{array}
    $
    

  \item[(update)]  $
    \begin{array}{llcl}
      (19) & \eval{\sql{update} R\; \sql{set} f''=e \;\sql{where}
  \phi}_v &  \coloneqq &  \sql{update} R\; \sql{set}
  f''=\eval{e}_v \;\sql{where}
  \eval{\phi}_v  \\
  (20) & \eval{\sql{update} R''\; \sql{set} f''=e \;\sql{where}
  \phi}_v &  \coloneqq &  \sql{update} R''\; \sql{set}
  f''=\eval{e}_v \;\sql{where}
  \eval{\phi}_v \\
%  (21) & \eval{\sql{update} R\; \sql{set} f=e \;\sql{where}
%  \phi}_v &\!\! \!\!\!\! \coloneqq & \!\!\! \!\!\!\sql{update} R'\; \sql{set} f'=\eval{e}_v \;\sql{where}
%  \param{\func{redirect}(\phi,v)}) \\
%  (22) & \eval{\sql{update} R\; \sql{set} f=e \;\sql{where}
%  \phi}_v & \!\!\! \!\!\! \coloneqq & \!\!\! \!\!\! \sql{update} R'\; \sql{set} \param{\func{duplicate}(f',\eval{e}_v)} \;\sql{where}
%  \param{\func{duplicate}(\eval{\phi}_v,v)})
    \end{array}
    $


\end{itemize}
\caption{Transformations triggered by a new value correspondence
$v=(R,R',f,f',\theta,\alpha)$}
  \label{fig:transformations}
\end{minipage}
%\end{mdframed}
\end{figure*}

\begin{lemma}
Given a program $P$, let $v=(R, R', f, f', \theta, \alpha)$ be a value correspondence and let $V = \mathcal{V}^{\func{id}}_{v,P}$. Then, if $(V_1,P) \hookrightarrow_{\textsc{v}} (V_1 \cup \{v\},P')$ and the refactoring semantics is equipped with the correct rewriting rules - which satisfy $R1$, $R2$ and $R3$, then $P' \preceq_V P$.
\end{lemma}
\begin{proof}
First we will show that for all histories $h' \in H(P')$, there exists a history $h \in H(P)$ such that $h' \preceq_{\mathcal{V}^{\func{id}}_{v,P}} h$. Given $h'$, the history $h$ is constructed by instantiating the same transactions as those in $h$ in the same order with the same arguments. Further, each command $\llbracket c \rrbracket_v$ of $P'$ executed in $h'$ corresponds to command $c$ of P. Hence, to construct the history $h$, we will execute the corresponding command for every execution step of $h'$. Formally, for a step $\Sigma'_1, \Delta'_1, \llbracket c \rrbracket_v \rightarrow \Sigma'_2, \Delta'_2, \llbracket c' \rrbracket_v$ in the history $h'$, we will perform the step $\Sigma_1, \Delta_1, c \rightarrow \Sigma_2, \Delta_2, c'$. We will show that the following invariant is maintained at every step: $\Sigma_2 \sqsubseteq_V \Sigma_2^{'}$, and $\Delta_2 \sqsubseteq_V \Delta_2^{'}$. We will use induction on the number of steps in the history $h'$ (which is same as the number of steps in history $h$). 

\textbf{Base Case}: In the beginning, both $\Sigma'$ and $\Delta'$ are empty. The first step in both $h$ and $h'$ is necessarily the application of the rule \textsc{txn-invoke}, which invokes an instance of some transaction $t$ in both $h$ and $h'$ with the same argument. Hence, after this step, both $\Sigma',\Delta'$ and $\Sigma,\Delta$ continue to remain empty and so the invariant holds trivially.

\textbf{Inductive Case}: Assume that the step $\Sigma_1^{'}, \Delta_1^{'}, \llbracket V,c_1 \rrbracket_v \rightarrow \Sigma_2^{'}, \Delta_2^{'}, \llbracket V,c_2 \rrbracket_v$ is performed in history $h'$ and the step $\Sigma_1, \Delta_1, c \rightarrow \Sigma_2, \Delta_2, c'$ is performed in the history $h$. By the inductive hypothesis, $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$, and $\Delta_1 \sqsubseteq_V \Delta_1^{'}$. We case split based on the type of step taken:

\textsc{txn-ret}: For a return expression $e$, by $(R2)$, since $\Delta_1 \sqsubseteq_V \Delta_1^{'}$, if $\Delta_1^{'}, \eval{e}_v \Downarrow n$, then $\Delta_1,e  \Downarrow n$. In this case, the corresponding transaction instances in $h$ and $h'$ return the same value $n$. Further, $\Sigma_2^{'} = \Sigma_1^{'}$, $\Delta_2^{'} = \Delta_1^{'}$ and $\Sigma_2 = \Sigma_1$, $\Delta_2 = \Delta_1$ and hence the invariant continues to hold. By similar reasoning, steps \textsc{cond-t}, \textsc{cond-f}, \textsc{iter} will also preserve the invariant.

\textsc{select}: We further case-split based on whether the $SELECT$ accesses the source field $f$ of the value correspondence $v$ or not. First, let us consider the case where the $SELECT$ accesses a different field. WLOG, let the command executed by $h'$ be $\eval{x:=\; \sql{select} f''\; \sql{from} {R''}\ \sql{where} \stx{\phi}}_v$. 

This is defined to be the command $x:=\; \sql{select} {f''}\; \sql{from} {R''}\ \sql{where}\eval{\phi}_v$. In $h'$, using the rule \textsc{consistent-view}, a view of the data store $\Sigma^{'*} \sqsubseteq \Sigma_1^{'}$ will be generated. Since the command accesses fields which are different from $f$, there are identity value correspondences for all the accessed fields in $V$, and since $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$, all the write events to fields accessed by the command in store $\Sigma_1^{'}$ will also be present in $\Sigma_1$. Hence, there exists a view $\Sigma^* \sqsubseteq \Sigma_1$ which contains the same write events to fields accessed by the command as $\Sigma^{'*}$. Finally, since $\Delta_1 \sqsubseteq_V \Delta_1^{'}$, by $(R2)$ all expressions $e$ present in the where clause $\phi$ will evaluate to same value in $h$ and $h'$. Hence, the same records will satisfy the where clauses $\eval{\phi}_v$ and $\phi$, leading to the same selection of records and hence the same binding to $x$, thus preserving $\Delta_2(x) \sqsubseteq_V \Delta_2^{'}(x)$.

Now, let us consider the case where the command executed by $h'$ is $\eval{V,x:=\; \sql{select} f\; \sql{from} {R}\ \sql{where} \stx{\phi}}_v$. This is defined to be the command $x:=\; \sql{select} {f'}\; \sql{from} {R'}\ \sql{where} \param{\func{redirect}(V,\eval{\phi}_v,v)}$.  In $h'$, using the rule \textsc{consistent-view}, a view of the data store $\Sigma^{'*} \sqsubseteq \Sigma_1^{'}$ will be generated to determine the records which satisfy the $WHERE$ clause $\func{redirect}(V,\eval{\phi}_v,v)$. Since $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$, for any record which satisfies $\func{redirect}(V,\eval{\phi}_v,v)$ and which is present in $\Sigma_1^{'}$, it corresponding record according to the value correspondence will also be present in $\Sigma_1$. Hence, we can construct a view of the data store $\Sigma^* \sqsubseteq \Sigma_1$ such that all fields of all records accessed in the $WHERE$ clause evaluate to the same value, i.e. $\Sigma^* \sqsubseteq \Sigma^{'*}$. Now, by $(R1)$, it is guaranteed that if records $\theta(r)$ are selected by $h'$, then the record $r$ must be selected by $h$. Further, since $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$ and $V$ includes the value correspondence $v$, the value of $f$ in the selected record in $h$ will satisfy the value correspondence $v$ w.r.t. the records $\theta(r)$ selected in $h'$. Hence, $\Delta_2(x) \sqsubseteq_V \Delta_2^{'}(x)$.

\textsc{update}: We case split based on whether the $UPDATE$ command modifies the source field $f$. First, let us consider the case where the $UPDATE$ modifies a different field. WLOG, let the command executed by $h$ be $\eval{\sql{update} R''\; \sql{set} f''=e \;\sql{where}\phi}_v$. This is defined to be the command $\sql{update} R''\; \sql{set} f''=\eval{e}_v \;\sql{where}\eval{\phi}_v$.

In $h'$, using the rule \textsc{consistent-view}, a view of the data store $\Sigma^{'*} \sqsubseteq \Sigma_1^{'}$ will be generated. Since the command accesses fields in the $WHERE$ clause which are different from $f$, there are identity value correspondences for all the accessed fields in $V$, and since $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$, all the write events to the accessed fields in store $\Sigma_1^{'}$ will also be present in $\Sigma_1$. Hence, there exists a view $\Sigma^* \sqsubseteq \Sigma_1$ which contains the same write events to the accessed fields as present in $\Sigma^{'*}$.  This guarantees that the same set of records in $R''$ will be selected by the $WHERE$ clauses in $h$ and $h'$ .Finally, since $\Delta_1 \sqsubseteq_V \Delta_1^{'}$, by $(R2)$, the expressions $\eval{V,e}_v$ and $e$ will evaluate to the same value. Hence, write events to the same field in the same set of records and writing the same value will be generated in $h$ and $h'$. This guarantees that $\Sigma_2 \sqsubseteq_V \Sigma_2^{'}$.

Now, let us consider the case where the command executed by $h'$ is $\llbracket \sql{update} R\ \sql{set} f=e\ \sql{where}\phi \rrbracket_v$. This is defined to be the command $ \sql{update} R'\ \sql{set} f' = \func{duplicate}(e,v)\ \sql{where} \func{duplicate}(\phi,v)$. n $h'$, using the rule \textsc{consistent-view}, a view of the data store $\Sigma^{'*} \sqsubseteq \Sigma_1^{'}$ will be generated to determine the records which satisfy the $WHERE$ clause $\func{duplicate}(\phi,v)$. Since $\Sigma_1 \sqsubseteq_V \Sigma_1^{'}$, if $\theta(r)$ is present in $\Sigma_1^{'}$, then $r$ would also be present in $\Sigma_1$. Hence, we can construct a corresponding view $\Sigma* \sqsubseteq \Sigma_1$ such that $\Sigma* \sqsubseteq_V \Sigma^{'*}$. Now, $(R3)$ guarantees that if any record in $\theta(r)$ is updated by $h'$, then the corresponding record $r$ would also be updated by $h$ (since it would satisfy the original $WHERE$ clause $\phi$). Further, $(R3)$ also guarantees the update $\func{duplicate}(e,v)$ in $h'$ would satisfy the value correspondence with the update in $h$. Hence, after the update $\Sigma_2 \sqsubseteq_V \Sigma_2^{'}$.

Note that the proof that for every serial execution of $P$, there exists an execution of $P'$ would follow the exact same pattern as above. In fact, we would actually construct a serial execution of $P'$ which would have the same behavior as the execution of $P$.
\end{proof}

\begin{lemma}
Given programs $P_1$, $P_2$ and $P_3$, a set of value-correspondences $V$ and a value correspondence $v$ such that the source and target fields of $v$ are not involved in any value correspondence in $V$, if $P_2 \preceq_{\mathcal{V}^{\func{id}}_{V,P_1} } P_1$ and $P_3 \preceq_{\mathcal{V}^{\func{id}}_{v,P_2}} P_2$, then $P_3 \preceq_{\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}} P_1$.
\end{lemma}
\begin{proof}
We are given $H_1: P_2 \preceq_{\mathcal{V}^{\func{id}}_{V,P_1} } P_1$ and $H_2:P_3 \preceq_{\mathcal{V}^{\func{id}}_{v,P_2}} P_2$. First we will show that for all histories $h \in H(P_3)$, there exists a history $h'' \in H(P_1)$ such that $h \preceq_{\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}} h''$. Let $h_{fin} = (\Sigma, \Gamma)$. By hypothesis $H_2$, there exists a history $h' \in H(P_2)$, $h' = (\Sigma', \Gamma')$ such that $\Gamma = \Gamma'$. By hypothesis $H_1$, there exists a history $h'' \in H(P_1)$, $h'' = (\Sigma'', \Gamma'')$ such that $\Gamma'' = \Gamma'$. Hence, $\Gamma'' = \Gamma$.

Now, by $H_2$, $H_3:\Sigma' \sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P_2}} \Sigma$, and by $H_1$, we have $H_4:\Sigma'' \sqsubseteq_{\mathcal{V}^{\func{id}}_{V,P_1}} \Sigma'$. We will show that $\Sigma'' \sqsubseteq_{\mathcal{V}^{\func{id}}_{V\cup\{v\},P_1}}$.

Consider a value correspondence $u \in V$, such that $u = (R,R',f,f',\theta, \alpha)$. Let $r \in R_\func{id}$. Suppose $r \in \Sigma''_{\func{id}}$. Then, by $H_4$, $\theta(r) \subseteq \Sigma'_\func{id}$. Now, since $f'$ is a field of $P_2$ which is not involved in value correspondence $v$, there exists an identity value correspondence $u' \in \mathcal{V}^{\func{id}}_{v,P_2}$, such that $u' = (R', R', f', f', \func{id}, \func{id})$. Hence, by $H_3$, we have $\theta(r) \subseteq \Sigma_\func{id}$. In the other direction, suppose $\theta(r) \subseteq \Sigma_\func{id}$. Then, by $H_3$, we have $\theta(r) \subseteq \Sigma'_\func{id}$, and hence by $H_2$, we have $r \in \Sigma''_{\func{id}}$.

Now, by $H_4$, $\Sigma''(r.f) = \alpha(\{m\ |\ r' \in \theta(r) \wedge \Sigma'(r'.f') = m\})$. By $H_3$ and the existence of the value correspondence $u'$, we have $\Sigma'(r'.f') = \Sigma(r'.f')$. Thus, $\Sigma''(r.f) = \alpha(\{m\ |\ r' \in \theta(r) \wedge \Sigma(r'.f') = m\})$.

Consider the value correspondence $v$ itself. Let $v = (R,R',f,f',\theta, \alpha)$. Since $f$ is not involved in any value correspondence in $V$, there exists an identity value correspondence $v'=(R,R,f,f,\func{id}, \func{id})$ such that $v' \in \mathcal{V}^{\func{id}}_{V,P_1}$. Let $r \in R_\func{id}$. Suppose $r \in \Sigma''_\func{id}$. Then by $H_4$, $r \in Sigma'_\func{id}$. By $H_3$, $\theta(r) \in \Sigma_\func{id}$. The other direction is straightforward. 

Now, by $H_3$, $\Sigma'(r.f) = \alpha(\{m\ |\ r' \in \theta(r) \wedge \Sigma(r'.f') = m\})$. By $H_4$, $\Sigma''(r.f) = \Sigma'(r.f)$. 

Hence, $\Sigma''(r.f) =  \alpha(\{m\ |\ r' \in \theta(r) \wedge \Sigma(r'.f') = m\})$.

Finally, consider an identity value correspondence in $\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}$ whose source field is neither in $V$ or in $v$. Then, this value correspondence is present in both $\mathcal{V}^{\func{id}}_{V,P_1}$ and $\mathcal{V}^{\func{id}}_{v,P_2}$. Hence, by $H_3$ and $H_4$, this value correspondence will also be preserved between $\Sigma''$ and $\Sigma$. Hence, $\Sigma'' \sqsubseteq{\mathcal{V\cup\{v\}}^{\func{id}}_{V,P_1}} \Sigma$. Thus, $h \preceq_{\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}} h''$.

Now we will show that for all histories $h'' \in H(P_1)_{\func{ser}}$, there exists a history $h \in H(P_3)_{\func{ser}}$ such that $h \preceq_{\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}} h''$. Let $h''_{fin} = (\Sigma'', \Gamma'')$, such that $h'' \in H(P_1)_{\func{ser}}$. By hypothesis $H_1$, there exists a history $h' \in H(P_2)_\func{ser}$, $h' = (\Sigma', \Gamma')$ such that $\Gamma'' = \Gamma'$ and $\Sigma'' \sqsubseteq_{\mathcal{V}^{\func{id}}_{V,P_1}} \Sigma'$. By hypothesis $H_2$, there exists a history $h \in H(P_3)_\func{ser}$, $h = (\Sigma, \Gamma)$ such that $\Gamma' = \Gamma$ and $\Sigma' \sqsubseteq_{\mathcal{V}^{\func{id}}_{v,P_2}} \Sigma$. Hence, $\Gamma'' = \Gamma$, and $\Sigma'' \sqsubseteq{\mathcal{V\cup\{v\}}^{\func{id}}_{V,P_1}} \Sigma$. Thus, $h \preceq_{\mathcal{V}^{\func{id}}_{V \cup \{v\},P_1}} h''$.
\end{proof}


\begin{theorem}
The refactoring semantics equipped with correct rewriting rules - which
satisfy $R1$, $R2$ and $R3$ - is sound, i.e.
    $ \forall_{P,P'}.\; \hstepc{\emptyset, P}{}{V, P'} \Rightarrow
    P'\preceq_{\mathcal{V}^{\func{id}}_{V,P}} P
$.
    \begin{proof}
Note that in order to express the result more formally, we have introduced new notation in the Appendix which has resulted in a slight change in the theorem statement from the main text of the paper. However, both statements signify the same result, since $V'$ used in the main text is actually the set of value correspondences introduced by the refactoring rules (same as $V$ in the above statement), and $\mathcal{V}^{\func{id}}_{V,P}$ contains $V$.

We first assume that all additions to the schema (either new relations or new fields) are carried out first using the rules \textsc{intro $\rho$} and \textsc{intro $\rho.f$}. These rules do not change the program, and since the original program $P$ is guaranteed to not access the new additions, it is clear that the statement of the theorem continues to hold after the above sequence of refactorings. Let $\func{Fld}_o$ be the set of all fields in the original program, and $\func{Fld}_n$ be the set of newly added fields. The rest of refactoring steps will involve multiple applications of the \textsc{intro $v$} rule. That is,
$$
(\emptyset,P) \hookrightarrow_{v_1} (\{v_1\}, P_1) \ldots \hookrightarrow_{v_n} (V,P_n)
$$
where $v_1, \ldots, v_n$ are the value correspondences that are introduced. We assume that the source field $f_i$ of every $v_i$ is a field of the original program i.e. $f_i \in \func{Fld}_o$ and the target field is a newly added field. We also assume that the no two value correspondences have the same source field or the same target field. Let $V = \{v_1, \ldots, v_n\}$. We will show that $P_n \preceq_{\mathcal{V}^{\func{id}}_{V,P}} P$. We will use induction on the number of refactoring steps ($n$). 

\textbf{Base Case}: For the first step, by applying Lemma B.1, $P_1 \preceq_{\mathcal{V}^{\func{id}}_{v_1,P_1}} P$.

\textbf{Inductive Case}: Assume that after $k$ steps, $P_k \preceq_{\mathcal{V}^{\func{id}}_{V_k,P_1}} P$, where $V_k = \{v_1, \ldots, v_k\}$. For the $(k+1)$th step $(V_k,P_k) \hookrightarrow_{v_{k+1}} (V', P_{k+1})$. Then, by Lemma B.1, $P_{k+1} \preceq_{\mathcal{V}^{\func{id}}_{v_{k+1},P_k}} P_k$. Now, by Lemma B.2, $P_{k+1} \preceq_{\mathcal{V}^{\func{id}}_{V_k \cup \{v_{k+1}\},P_1}} P_1$.  
\end{proof}
  \end{theorem}
  
\begin{theorem}
  The rewrite rules described in this section (i.e. by (I1.1), (I1.2),
  (I2.1), (I2.2), (I3.1) and (I3.2))
  satisfy the correctness properties (R1), (R2) and (R3).
    \begin{proof}
We will first show that (I1.1) satisfies (R1). We are given a value correspondence $v=(R,R',f,f',\theta,\alpha)$. Let $V = \mathcal{V}^{\func{id}}_{v,P}$. The value correspondence $v$ satisfies the property that $\alpha = \func{any}$ and $\theta$ selects records in $R'$ based only equality predicates on all the primary-key fields of $R$. Assume that each primary key field $p \in R_{\func{pk}}$ is equated with expression $e_p$ in the where clause $\phi$. Given $\Sigma, \Sigma', \Delta, \Delta'$ such that $\Sigma \sqsubseteq \Sigma'$ and $\Delta \sqsubseteq \Delta'$, consider $r \in R_\func{id}$. Assume that $\Delta, e_p \Downarrow n_p$. By (R2), we have $\Delta, e_p \Downarrow n_p$. Suppose $r \in \Sigma_\func{id}$.

\begin{align*}
\Delta,\phi(\Sigma(r))\Downarrow \func{true} & \Rightarrow \bigwedge_{p \in R_\func{pk}} \Sigma(r.p) = n_p
\end{align*}

This in turn implies that $\theta(r) = \{r'\ |\ r' \in R'_\func{id} \wedge \forall p \in R_\func{pk}. \Sigma'(r'.\hat{\theta}(p)) = n_p\}$. Since $\Sigma \sqsubseteq_V \Sigma'$, at least one such record in $\theta(r)$ is also present in $\Sigma'$. Now, by definition of $\func{redirect}(v,\phi)$,

\begin{align*}
r' \in \Sigma' \wedge \Delta',{\func{redirect}(v,\phi)}(\Sigma'(r')) \Downarrow \func{true}\} \Rightarrow \bigwedge_{p \in R_\func{pk}} \Sigma'(r'.\hat{\theta}(p)) = n_p
\end{align*}

We have just shown that at least one such record is guaranteed to be present in $\Sigma'$, and hence the intersection of $\theta(r)$ and above set is non-empty. To prove the reverse direction, we follow the same steps in reverse order. Since $\func{redirect}$ picks exactly the records which satisfy the above condition, the containment relation $\Sigma \sqsubseteq_V \Sigma'$ guarantees that $\Sigma'(r'.f') = \Sigma(r.f)$. This completes the proof that (I1.1) satisfies (R1). 

Now we will show that (I2.1) satisfies (R2). Consider the simple expression $e = \func{at}^1(x.f)$. Since $\Delta(x) \sqsubseteq \Delta'(x)$, there exists at least one record bound to $x$ in $\Delta'$. Further,  the value at field $f'$ in this record must be equal to the value at field $f$ of any record bound to $x$ in $\Delta$. Hence, $\func{at}^1(x.f) = \func{at}^1(x.f')$. Thus, (R2) follows for $e$. For compound expressions, the proof directly follows using induction on the structure of the expression.

Now we will show that (I3.1) satisfies (R3). The first condition in the goal of (R3) is the same as the first condition in goal of (R1). Due to (R2), the second condition also directly holds.

Now, we will prove the results about the logger refactoring. Note that this for $SELECT$ statement and expression transformations, this refactoring uses the same $\func{redirect}$ definition as above. Hence, the above proofs for (R1) and (R2) directly apply in this case for (I1.2) and (I2.2). Let us now prove that (I3.2) satisfies (R3). The first condition in the antecedent of (R3) holds directly by the same reasoning as applied in the cases above. For the second condition, note that due to the $\func{sum}$ value correspondence, the following holds:

\begin{align*}
\Sigma(r.f) = \sum_{r' \in \theta(r) \cap \Sigma'_\func{id}} \Sigma(r'.f')
\end{align*}

Assuming that $\Delta, e \Downarrow n$ (also $\Delta', e \Downarrow n$ due to (R2)), the updated value in record $r$ satisfying $\phi$ would be $\Sigma(r.f) + n$. On the R.H.S, a new record in $\theta(r)$ would be added in $\Sigma''$, with the value in the field $f'$ being $n$. Thus, the same value is added on both sides of the above equation, resulting in equal values again. This completes the proof that (I3.2) satisfies (R3). 
  \end{proof}
\end{theorem}


==> sections/case.tex <==
\section{Case study: tpc-c}


==> sections/refactor.tex <==
\section{Repair procedure}
\label{sec:ref}





==> sections/search.tex <==
\newpage
\section{Search Space and Algorithm}
\label{sec:search}



%------------------------------
\subsection{Serializability Anomalies and NAAs}


\subsubsection{FOL Encoding}

%------------------------------
\subsection{Search Algorithm}











==> sections/semantics.tex <==
\section{Semantics of Database Programs Refactoring}
\label{sec:semantics}

%------------------------------
\subsection{Database Programs}
%------------------------------

\input{figures/schema_syntax}
\input{figures/program_syntax}


%------------------------------
\newpage
\subsection{Refactoring Syntax and Semantics}
%------------------------------

\input{figures/schema_modification_syntax}
%\input{figures/schema_function_definitions}
\input{figures/schema_modification_semantics_top}
\input{figures/schema_modification_semantics_chsk}
\input{figures/schema_modification_semantics_id}
\input{figures/schema_modification_semantics_sum}
\input{figures/program_shrinking_semantics}
\input{figures/program_shrinking_semantics_merge}
\input{figures/program_shrinking_semantics_redirect}















==> sections/ser.tex <==
\newpage
\newpage
\section{Eventual Consistency and Serializability Anomalies}
\label{sec:ser}
\subsection{EC semantics}
\begin{itemize}
  \item Read and write effects 
  \item $ar$ and $vis$ between effects
  \item Database state $\mathcal{I}$
  \item Equivalence on database states
    $\mathcal{I}\equiv\mathcal{I}'$ (of isomorphic schemas)
  \item Introduce $\mathcal{I}\xrightarrow{EC} \mathcal{I}'$ operational semantics
  \item Bounded observational equivalence $P\equiv^b P'$ and refinement
    $P'\preceq^b P$ between
    isomorphic programs
\end{itemize}


\subsection{Serializability Anomalies}
\begin{itemize}
  \item Introduce dependency relations between queries
  \item Define serializability anomalies
  \item Define (anomalous) data access instances $\alpha$
  \item Define isomorphism on $\alpha$ and containment between sets of $\alpha$
  \item Introduce the bounded anomaly detection oracle, $\mathcal{O}^b$,
    and define its properties
\end{itemize}




